Stochastic Robustness Interval for Motion Planning with Signal Temporal Logic

In this work, we present a novel robustness measure for continuous-time stochastic trajectories with respect to Signal Temporal Logic (STL) specifications. We show the soundness of the measure and develop a monitor for reasoning about partial trajectories. Using this monitor, we introduce an STL sampling-based motion planning algorithm for robots under uncertainty. Given a minimum robustness requirement, this algorithm finds satisfying motion plans; alternatively, the algorithm also optimizes for the measure. We prove probabilistic completeness and asymptotic optimality, and demonstrate the effectiveness of our approach on several case studies.

==> ICRA23_sections/Experiments.tex <==
\section{Evaluations}
We evaluate efficacy and efficiency of the proposed measure and planners subject to a variety of STL specifications. The algorithms are implemented with \X= RRT \cite{RRT}, i.e., \stori-RRT. The hyperparameters of our algorithm used in each case study are provided in \cite{Ilyes2022extended}. All algorithms are implemented in the Open Motion Planning Library (OMPL)~\cite{sucan2012the-open-motion-planning-library}, and computations were performed on 3.9 GHz CPU and 64 GB of RAM. 

We considered a noisy second-order unicycle system whose stochastic dynamics are given by:
% \begin{equation}
% \label{eq:unicycle}
    $dx = v \cos(\theta) dt + dw$, 
    $dy = v \sin(\theta) dt + dw$,
    $d\theta = u_\omega dt + dw$,
    $dv = u_a dt + dw$
% \end{equation}
where $u_a$ and $u_\omega$ are the acceleration and steering angle inputs. We linearized the dynamics according to the feedback linearization in \cite{unicycle}.  We considered environments in Figs. \ref{fig:examples}, \ref{fig:form2}, and \ref{fig:form4} respectively  with STL formulae $\varphi_1$ in \eqref{eq:form1}, 
\begin{align}
    \varphi_2 &= \lnot O U_{[0,10]} A \land \lnot O U_{[0,10]} B, \label{eq:form2}\\
    % &W = x \geq 0 \land x \leq 4 \land y \geq -2 \land y \leq 2 \notag\\
    &O = x \geq 1.5 \land x \leq 3.5 \land y \geq -0.5 \land y \leq 0.5, \notag\\
    &A = x \geq 2 \land x \leq 3 \land y \geq 1, \notag\\
    &B = x \geq 2 \land x \leq 3 \land y \leq -1, \notag
    \end{align}
    \begin{align}
    \varphi_3 &= (\text{Puddle} \rightarrow \lnot \text{Charge} U_{[0,3]} \text{Carpet}) U _{[0,10]} \text{Charge}, \label{formeq:3}\\
    &\text{Puddle} = y \leq 2.5 \land x \geq 2 \land x \leq 3, \notag\\
    &\text{Charge} = y \geq 2 \land x \geq 4, \notag\\
    &\text{Carpet} = y \leq 1 \land x \geq 4. \notag
\end{align}
% $\text{Charge} = y \geq 2 \land x \geq 4$, and $\text{Carpet} = y \leq 1 \land x \geq 4$.
Here, $\varphi_2$ requires avoiding (black) region $O$ until both regions $A$ and $B$ are visited within 10 minutes in Fig. \ref{fig:form2}. $\varphi_3$ requires the robot to go to the charger within 10 minutes and also that, if it visits the puddle, it must avoid the charger until it visits the carpet within 3 minutes of visiting the puddle in Fig. \ref{fig:form4}. For all formulas, we also require the robot to remain in the workspace for the duration of the mission. 

\subsection{Case Study 1 - Computation Time vs \stori Threshold}

This case study seeks to analyze the relationship between computation time and the \storm constraint $\kappa$. Specifically, we study how \stori-RRT performs 
% when planning motions for system \ref{eq:unicycle} subject to STL 
for formula $\varphi_2$, in the environment in Fig. \ref{fig:form2}. 
We ran $100$ trials, with a maximum computation time of $300$ seconds for each trial. 
Table \ref{tab:bench1} reports the computation time and success rate for different $\kappa$ values. We see that computation time increases and success rate decreases as the $\kappa$ threshold increases. This is due to the increased difficulty of satisfying the robustness constraint.

\begin{table}[h]
    \centering
    \caption{Benchmarking Results for Case Study 1}
    \begin{tabular}{|c|c|c|}
    \hline
        \storm Threshold $\kappa$ & Computation Time (s) & Success Rate\\ 
        \hline
        0.50 & 60.10 $\pm$ 64.87 & 97\%\\
        0.70 & 71.37 $\pm$ 67.48 & 97\%\\
        0.90 & 83.30 $\pm$ 69.35 & 90\%\\
        0.95 & 92.48 $\pm$ 81.56 & 86\%\\
        \hline
    \end{tabular}
    \label{tab:bench1}
    % \vspace{-3mm}
\end{table}

Fig. \ref{fig:form2} shows two sample trajectories for this specification, where the ellipses represent the 90\% confidence
bounds of their uncertainty. Trajectory 1 uses $\kappa = 0.9$ and goes through the wider opening on the left. In contrast, Trajectory 2 uses $\kappa = 0.5$ and finds less robust paths that go through the narrow opening on the right. 

\begin{figure}[t]
\centering
\begin{subfigure}{0.235\textwidth}
    \centering
    \includegraphics[width=\linewidth,trim={1cm 0cm 2cm 0cm},clip]{figures/form2.eps}
    \caption{$\phi_2$ Trajectories}
    % \caption{Two Trajectories for formula $\phi_2$. Trajectory 1 has a \stori of [0.944,0.991] and trajectory 2 has a \stori of [0.78,0.781]}
    \label{fig:form2}
\end{subfigure}
\begin{subfigure}{0.235\textwidth}
    \centering
    \includegraphics[width = \linewidth,trim={1cm 0 2cm 0},clip]{figures/bench3.eps}
    \caption{Case Study 3 Benchmark}
    \label{fig:case3}
\end{subfigure}
\caption{Experiment Results. (a) shows two trajectories where $\low{f}(\varphi_2,\btraj_1) = 0.98, \low{f}(\varphi_2,\btraj_2) = 0.67$, and (b) shows benchmarking results for Case Study 3.}
\label{fig:results}
\vspace{-3mm}
\end{figure}



\subsection{Case Study 2 - Computation Time for Different Formulas}
This case study compares computation time for different STL formulas. Table \ref{tab:bench2} shows the average computation time of \stori-RRT for the three formulas and environments over 100 trials with a maximum timeout of 300s. We used \storm bound $\kappa = 0.9$. We see that, even with a tight \storm threshold $\kappa$, the algorithm finds solutions with a good success rate and computation time. This shows that the algorithm is generally applicable to all STL formulas. 

\begin{table}[t]
    \caption{Benchmarking Results for Case Study 2, $\kappa = 0.9$.}
    \label{tab:bench2}
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
        Formula & Computation Time (s) & Success Rate\\ 
        \hline
        $\varphi_1$ & 1.98 $\pm$ 2.56 & 100\%\\
        $\varphi_2$ & 85.95 $\pm$ 82.56 & 90\%\\
        $\varphi_3$ & 44.55 $\pm$ 53.89 & 99\%\\
        \hline
    \end{tabular}
     \vspace{-3mm}
\end{table}

\subsection{Case Study 3 - Asymptotic Optimality}
In this case study, we analyze the relationship between given computation time and the \storm of the resulting trajectory. Here, we study how AO-\stori-RRT performs when planning for formula $\varphi_3$, in the environment in Fig. \ref{fig:form4}. Fig. \ref{fig:case3} presents the results of 100 trials. It clearly shows that the solutions asymptotically approach an optimal \storm. Fig. \ref{fig:form4} gives two sample trajectories with different {\storm}s. Trajectory 2 is found earlier in the optimization, and makes it through the gap. When the planner further optimizes for the \storm, however, it favors trajectories like Trajectory 1, that enter the puddle and dry off before going to the carpet. 

\subsection{Case Study 4 - Simulated Performance}
This case study seeks to analyze how the \storm relates to the \textit{statistical satisfaction rate} (SSR) defined as $\frac{\#\text{satisfying runs}}{\text{total \# runs}}$. We do this by simulating the robot's motion plans from \stori-RRT. Table \ref{tab:corr} compares the \stori of the belief trajectories against the 
% statistical satisfaction rate 
SSR
of the simulated realizations. Each motion plan is simulated 1000 times. We use the Breach Toolbox \cite{rosi} to evaluate the realizations' satisfaction. These results show correlation between the \storm  and probability of satisfaction.

\begin{table}[ht]
    % \caption{Comparison of StoRI and statistical satisfcation rate for controllers synthesized with StoRI-RRT
    \caption{Comparison of StoRI against SSR
    }
    \label{tab:corr}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        Formula & $\low{f}(\phi,\btraj)$ (\storm) & $\up{f}(\phi,\btraj)$ & Satisfaction Rate\\
        \hline
        $\varphi_1$ & 0.568 & 0.568  & 0.367\\
        $\varphi_1$ & 0.755 & 0.781  & 0.767\\
        $\varphi_1$ & 0.986 & 0.986  & 0.985\\ 
        \hline
        $\varphi_2$ & 0.572 & 0.589  & 0.582\\
        $\varphi_2$ & 0.873 & 0.998  & 0.754\\
        $\varphi_2$ & 0.912 & 0.913  & 0.889\\
        \hline
        $\varphi_3$ & 0.625 & 0.677  & 0.669\\ 
        $\varphi_3$ & 0.876 & 0.878  & 0.872\\
        $\varphi_3$ & 0.989 & 0.994  & 0.985\\
        \hline
    \end{tabular}
     \vspace{-3mm}
\end{table}



==> ICRA23_sections/Methodology.tex <==
\section{Motion Planning Algorithm}
\label{sec:motion-planning}
This section presents two sampling-based motion planners that utilize \stori and the \stori Monitor. The first planner finds solutions that satisfy a given \storm constraint, and the second finds solutions that directly optimize for the \storm. 

\subsection{StoRI-\X}
A kinodynamic sampling-based tree planner \X grows a motion tree in the state space $X$ according to the robot dynamics through sampling and extension procedures. 
We generalize planner \X to \stori-\X (Alg. \ref{alg:StoRIX}) to generate plans for System~\eqref{eq:SDE} that are guaranteed to satisfy a given lower bound $\kappa \in [0,1]$ on \storm with respect to STL formula $\phi$.  
% \stori-\X planner is outline in Alg. \ref{alg:StoRIX}.
% \ri{to-do: clearly introduc $N$ and $\kappa$}
% \qh{This feels unnecessary}
% \ri{yo, I'm inclined to agree; $\kappa$ is casually defined in this paragraph and N is mentioned in the explanation below. @Morteza, can we ignore this comment?}

\begin{algorithm}
\caption{\stori-\X$(X,U,\phi,\hat{x}_0,N,\kappa)$}
\label{alg:StoRIX}
$P_0 \gets 0^{n \times n}$\;
$\mathbb{V} \gets \{(\ha
t{x}_0,P_0)\},\mathbb{E} \gets \emptyset $\;
$\mathbb{G} \gets \{\mathbb{V},\mathbb{E}\}$\;
\For{N iterations}{
    $\hat{x}_{rand},t_{rand},\hat{x}_{near},P_{near} \gets sample(X,\mathbb{V},T)$\;
    $\hat{x}_{new},P_{new} \gets $ Extend($\hat{x}_{near},P_{near},U$)\;
    \If{$\up{\Tilde{f}}(\phi,(\hat{x}_0,P_0)...(\hat{x}_{new},P_{new})) > \kappa$}{
        $\mathbb{V} \gets \mathbb{V} \cup \{(\hat{x}_{new},P_{new})\}$ \;
        $\mathbb{E} \gets \mathbb{E} \cup \{[(\hat{x}_{near},P_{near}),(\hat{x}_{new},P_{new})]\}$\;
        \If{$\low{f}(\phi,(\hat{x}_0,P_0)...(\hat{x}_{new},P_{new})) > \kappa$}{
            \Return $(\hat{x}_0,P_0)...(\hat{x}_{new},P_{new})$\;
        }
    }
}
\Return $\emptyset$ %\mathbb{G}$
\end{algorithm}


% It takes the state space $X$, input space $U$, STL formula $\phi$, the initial state $\hat{x}_0$, the number of iterations $N$, and the user-specified stochastic robustness constraint $\kappa$\ri{Are the plant dynamics/noise diffusion matrix also inputs?}. The algorithm returns a motion plan that satisfies the constraint, if found within $N$ iterations. \qh{This part from 'It takes... ' are already written as inputs in the algorithm}

The algorithm first initializes the tree $\mathbb{G}$ with the belief of $x(0)$. Each node in this tree is a tuple $(\hat{x},P)$ of the mean and covariance of the distribution that describes the state. At every iteration, the algorithm samples a random state $\hat{x}_{rand}$ and time $t_{rand}$ and computes the nearest existing node $(\hat{x}_{near},P_{near})$. $t_{rand}$ is sampled from the time-horizon of the STL formula as defined in \cite{rosi}, and the nearest node is selected using a distance metric that accounts for both state distance $\|\hat{x}_{rand} - \hat{x}_{near}\|$ and time distance $|t_{rand} - t_{near}|$. Second, a random control input $u \in U$ and time duration $t$ is sampled and propagate the system from $(\hat{x}_{near},P_{near})$ to generate a new belief node $(\hat{x}_{new},P_{new})$. Third, the \stori Monitor of the partial belief trajectory $\ptraj = (\hat{x}_0,P_0)(\hat{x}_1,P_1)\cdots(\hat{x}_{new},P_{new})$ is computed for the formula $\phi$. If the \stori Monitor has an upper bound $\up{\Tilde{f}}(\phi,\ptraj) \leq \kappa$, $\ptraj$ has already violated the STL Specification and the new node is discarded. Otherwise, we add $(\hat{x}_{new},P_{new})$ and the edge $\big((\hat{x}_{near},P_{near}),(\hat{x}_{new},P_{new})\big)$ to $\mathbb{G}$. Finally, $\ptraj$ is a solution if the \storm $\low{f}(\phi,\ptraj) > \kappa$. This process repeats until a solution is found or for a maximum of $N$ iterations.

% We first initialize the graph with the initial state and a zero covariance matrix. At every iteration, we sample a random state $\hat{x}_{rand}$ and time $t_{rand}$ and find the nearest existing node $(\hat{x}_{near},P_{near})$. The time is sampled from the time-horizon of the STL formula \ri{how better to say this without needing definition?}, and is weighed in the distance when selecting a near node. We then sample a random control input $u \in U$ and time duration $t$ and propagate the system from $(\hat{x}_{near},P_{near})$ to generate a new belief $(\hat{x}_{new},P_{new})$. The algorithm then calculates the \stori Monitor of the partial belief trajectory $\ptraj = (\hat{x}_0,P_0)(\hat{x}_1,P_1)\cdots(\hat{x}_{new},P_{new})$ with respect to the formula $\phi$. If the \stori monitor has an upper bound $\up{\Tilde{f}}(\phi,\ptraj) < \kappa$, the partial trajectory has already violated the STL Specification and the new node is not added to the tree. Otherwise, we add the vertex $(\hat{x}_{new},P_{new})$ and the edge $[(\hat{x}_{near},P_{near}),(\hat{x}_{new},P_{new})]$ to $\mathbb{G}$. The partial trajectory is a solution if the lower bound $\low{\Tilde{f}}(\phi,\ptraj) > \kappa$. This process repeats until a solution is found or for a maximum of $N$ iterations.
% This section presents Fast Random Optimal StoRI Trees (FROST), a planning algorithm that finds motion plans for stochastic systems that satisfy a user-specified threshold on the lower bound of the StoRI of the resulting trajectory with respect to an STL formula $\phi$. \ri{I'd like to use the name GHOST if we can think of something for H (G would be 'Gaussian')}
\begin{theorem}[Probabilistic Completeness]
\label{theorem:complete}
Planner \stori-\X in Alg.~\ref{alg:StoRIX} is probabilistically complete if the underlying planner \X is probabilistically complete.
\end{theorem}
\begin{proof}[Proof]
    \stori-\X mimics the behavior of planner \X, only modifying its validity check. From Theorem \ref{theorem:monitorbounds}, this modification only rejects nodes that are guaranteed to violate the STL Specification $\phi$. Therefore, if a solution exists, \stori-\X will find it with probability $1$ as $N \rightarrow \infty$. 
\end{proof}


% \ri{todo: find reach regions once at beginning of AO version}
% \begin{algorithm}[h]
% \caption{StoRI-RRT($X,U,N,\hat{x}_0,P_0,\kappa, \phi, \mathcal{R})$}
% \label{alg:RRT}
% $\mathbb{V} \gets \{(\hat{x}_0,P_0)\}$;
% $\mathbb{E} \gets \emptyset, \mathbb{G} \gets \{\mathbb{V},\mathbb{E}\}$\;
% \For{$n = 1$ to $N$}
% {
%     $t_{sample} \gets$ TimeSample($\mathbb{T}$)\;
%     $x_{sample} \gets$ ReachSample($\mathcal{R},t_{sample}$)\;
%     $x_{near} \gets$ BestNear($\mathbb{V}_{active},x_{sample},\delta v$)\;
%     $u_{sample} \gets$ SampleControl($U$)\;
%     $t_{prop} \gets$ Uniform(0,$\mathbb{T}$)\;
%     $x_{new},P_{new} \gets$ Propagate($x_{near},u_{sample},t_{prop}$)\;
%     $I \gets$ FindStoRI($x_0 \rightarrow x_{new}, \phi$)\;
%     \If{$\up{I} \geq \kappa$} {
%         $\mathbb{V} \gets \mathbb{V} \cup \{(x_{new},P_{new})\}$ \;
%         $\mathbb{E} \gets \mathbb{E} \cup \{x_{near} \rightarrow x_{new}\}$\;
%         \If{$\low{I} \geq kappa$}{
%         break\;
%         }
%     }
% }
% \Return $(\mathbb{G},n,\low{I})$\;
% \end{algorithm}



% \begin{algorithm}[h]
% \caption{FROST($X,U,\hat{x}_0,P_0,dt,N,\delta_v, \delta_s,\kappa, \phi)$}
% \label{alg:StSST}
% $i \gets 0$\;
% $\mathbb{V}_{active} \gets \{(\hat{x}_0,P_0)\}$, $\mathbb{V}_{inactive} \gets \emptyset$\;
% $\mathbb{V} \gets \mathbb{V}_{active} \cup \mathbb{V}_{inactive}$\;
% $\mathbb{E} \gets \emptyset, \mathbb{G} \gets \{\mathbb{V},\mathbb{E}\}$\;
% $s_0 \gets x_0, s_0.rep = x_0, S \gets \{s_0\}$\;
% $\mathcal{R} \gets$ FindReachRegions($\phi,\emptyset,\top,[0,0]$)\;
% \While{$N \neq 0$}
% {
%     $t_{sample} \gets$ TimeSample($\mathbb{T}$)\;
%     $s_{sample} \gets$ ReachSample($\mathcal{R},t_{sample}$)\;
%     $x_{nearest} \gets$ BestNear($\mathbb{V}_{active},s_{sample},\delta v$)\;
%     $u_{sample} \gets$ SampleControl($U$)\;
%     $x_{new} \gets$ Propagate($x_{nearest},u_{sample},dt$)\;
%     $I \gets$ FindStoRI($x_0 \rightarrow x_{new}, \phi$)\;
%     \If{$\lceil I \geq \kappa$} {
%         $s_{new} \gets$ Nearest($S,x_{new}$)\;
%         \If{$dist(x_{new},s_{new}) > \delta_s$} {
%             $S \gets S \cup \{x_{new}\}$\;
%             $s_{new} \gets x_{new}$\;
%             $s_{new}.rep \gets NULL$\;
%         }
%         $x_{peer} \gets s_{new}.rep$\;
%         \If{$x_{peer} == NULL$ or cost($x_{new}) <$ cost($x_{peer}$)} {
%             $\mathbb{V}_{active} \gets \mathbb{V}_{active} \symbol{92} \{x_{peer}\}$\;
%             $\mathbb{V}_{inactive} \gets \mathbb{V}_{inactive} \cup \{x_{peer}\}$ \;
%             $s_{new}.rep \gets x_{new}$\;
%             $\mathbb{V}_{active} \gets \mathbb{V}_{active} \cup \{x_{new}\}$ \;
%             $\mathbb{E} \gets \mathbb{E} \cup \{x_{nearest} \rightarrow x_{new}\}$\;
%             \While{IsLeaf($x_{peer}) \land x_{peer} \in \mathbb{V}_{inactive}$} {
%                 $\mathbb{E} \gets \mathbb{E} \symbol{92} \{x_{parent} \rightarrow x_{peer}\}$\;
%                 $\mathbb{V}_{inactive} \gets \mathbb{V}_{inactive} \symbol{92} \{x_{peer}\}$\; 
%                 $x_{peer} \gets x_{parent}$\;
%             }
%         }
%     }
% }
% \Return %$\mathbb{G}$\;
% \end{algorithm}

\subsection{Asymptotically Optimal StoRI-\X (AO-StoRI-\X)}
Since the \storm allows us to compute a quantitative value of robustness, we can also optimize for the \storm of a belief trajectory in a sampling-based motion planner. This is enabled through the AO-$\mathcal{A}$ meta-algorithm in \cite{ao-rrt}, by repeatedly calling \stori-\X with increasing $\kappa$ bounds by setting $\kappa$ as the \storm of the previous solution at 
each iteration \cite{Ilyes2022extended}.


% Since the \storm allows us to compute a quantitative value of robustness, we can also optimize for the \storm of a belief trajectory in a sampling-based motion planner. This is enabled through the AO-$\mathcal{A}$ meta-algorithm in \cite{ao-rrt}, by repeatedly calling \stori-\X with increasing $\kappa$ bounds by setting $\kappa$ as the \storm of the previous solution at each iteration \cite{Ilyes2022extended}.


% %%%%%%%%%%%%%%%%%
% \begin{algorithm}
% \caption{AO-StoRI-\X($X,U,\phi,\hat{x}_0,N)$)}
% \label{alg:frost}
% $\kappa \gets 0$\;
% \While{$N \neq 0$}{
% $\btraj,n \gets $StoRI-\X($X,U,\phi,\hat{x}_0,N,\kappa)$)\;
% $\kappa \gets \low{f}(\phi,\btraj)$\; 
% $N \gets N - n$\;
% }
% \Return $\btraj$ if solution found, No Solution otherwise
% % \ri{do we just return the tree if we run out of time/iterations??}\qh{I think it's fine as is}
% \end{algorithm}

% The algorithm is summarized in Alg.~\ref{alg:frost}.
% Here, we present Fast Robustly-Optimal StoRI Trees (FROST), a motion planner that iteratively optimizes \storm of belief trajectories. The algorithm is built upon the Asymptotically Optimal Rapidly Exploring Random Trees (AO-RRT) algorithm \cite{ao-rrt}. FROST returns the motion plan with the highest \storm for the STL formula after $N$ iterations. It repeatedly calls StoRI-X (Alg.~\ref{alg:StoRIX}) while iteratively increasing $\kappa$, optimizing the \storm of the final trajectory $\btraj$. Line $1$ of Alg.~\ref{alg:frost} initializes this robustness constraint to $0$. The algorithm first finds an initial solution using StoRI-X (line 2), with its corresponding \storm. Then, at every iteration, the algorithm sets $\kappa$ to the new found \storm of the previous solution, and finds a new solution with this new constraint.
% \begin{algorithm}
% \caption{FROST($X,U,N, M, \hat{x}_0,P_0,\phi)$)}
% \label{alg:frost}
%     $\kappa \gets 0$\;
%     % $\mathcal{R} \gets$ FindReachRegions($\phi,\emptyset,\top,[0,0]$)\;
%     $\btraj \gets $StoRI-X($X,U,M,\hat{x}_0,P_0,\kappa,\phi,\mathcal{R}$)\;
%     $\kappa \gets \low{f}(\phi,\btraj)$\;
%     \For{$N$ iterations}{
%     %\While{$N \neq 0$}{
%         $\btraj \gets $StoRI-RRT($X,U,M,\hat{x}_0,P_0,\kappa,\phi$)\;
%         $\kappa \gets \low{f}(\phi,\btraj)$\;
%         %$N \gets N - n$\;
%     }
%     \Return $\btraj$ if solution found, No Solution otherwise
% % \ri{do we just return the tree if we run out of time/iterations??}\qh{I think it's fine as is}
% \end{algorithm}
% \begin{algorithm}
% \caption{AO-StoRI-X($X,U,N,\hat{x}_0,P_0,\phi)$)}
% \label{alg:frost}
% $\kappa \gets 0$\;
% % $\mathcal{R} \gets$ FindReachRegions($\phi,\emptyset,\top,[0,0]$)\;
% $\btraj,n \gets $StoRI-X($X,U,N,\hat{x}_0,P_0,\kappa,\phi,\mathcal{R}$)\;
% $\kappa \gets \low{f}(\phi,\btraj)$\;
% $N \gets N - n$\;
% \While{$N \neq 0$}{
% $\btraj,n \gets $StoRI-RRT($X,U,N,\hat{x}_0,P_0,\kappa,\phi$)\;
% $\kappa \gets \low{f}(\phi,\btraj)$\; 
% $N \gets N - n$\;
% }
% \Return $\btraj$ if solution found, No Solution otherwise
% % \ri{do we just return the tree if we run out of time/iterations??}\qh{I think it's fine as is}
% \end{algorithm}
% \begin{proposition}[Asymptotically Optimal]
%     \label{theorem:optimal}
%     Planner AO-StoRI-X in Alg.~\ref{alg:frost} is asymptotically optimal if the underlying planner X is well-behaved. 
% \end{proposition}
% The algorithm is built upon the Asymptotically Optimal Rapidly Exploring Random Trees (AO-RRT) algorithm \cite{ao-rrt}. FROST returns the motion plan with the highest \storm for the STL formula after $N$ iterations. It repeatedly calls StoRI-X (Alg.~\ref{alg:StoRIX}) while iteratively increasing $\kappa$, optimizing the \storm of the final trajectory $\btraj$. Line $1$ of Alg.~\ref{alg:frost} initializes this robustness constraint to $0$. The algorithm first finds an initial solution using StoRI-X (line 2), with its corresponding \storm. Then, at every iteration, the algorithm sets $\kappa$ to the new found \storm of the previous solution, and finds a new solution with this new constraint.
% Therefore, we initialize $\kappa = 0.5$. \qh{this sentence still seems redundant}
%%%%%%%%%%%%%%%%%%%%%%%%% Old supplementary algos related to heuristic
% \begin{algorithm}
% \caption{FindReachRegions($\phi,\mathcal{R},reachflag,[t_1,t_2]$)}
% \label{alg:findRegions}
% \uIf{$\phi \in \{\top,\bot\}$}{
% \Return $\mathcal{R}$\;
% }
% \uElseIf{$\phi = \mu \land reachflag$}{
% \Return $\mathcal{R} \cup (\phi,[t_1,t_2])$\;
% }
% \uElseIf{$\phi = \phi_1 \land \phi_2$}{
% \uIf{IsConjunctionTree($\phi$)}{
% \uIf{$reachflag$}{
% \Return $\mathcal{R} \cup (\phi,[t_1,t_2])$\;
% }
% \uElse{
% \Return $\mathcal{R}$\;
% }
% }
% \uElse{
% FindReachRegions($\phi_1,\mathcal{R},reachflag,[t_1,t_2]$)\;
% FindReachRegions($\phi_2,\mathcal{R},reachflag,[t_1,t_2]$)\;
% }
% }
% \uElseIf{$\phi = \lnot \phi '$}{
% $reachflag = \lnot reachflag$\ri{does this make sense? flip the reach flag}\;
% FindReachRegions($\phi ',\mathcal{R},reachflag,[t_1,t_2]$)\;
% }
% \uElseIf{$\phi = \phi_1 U_{[a,b]} \phi_2$}{
% FindReachRegions($\phi_1,\mathcal{R},reachflag,[a,b]$)\;
% FindReachRegions($\phi_2,\mathcal{R},reachflag,[a,b]$)\;
% \ri{believe i need to adjust this to make sure it's correct for nested formulas as well}
% } 
% \end{algorithm}

% \begin{algorithm}
% \caption{IsConjunctionTree($\phi$)}
% \label{alg:conjTree}
% \uIf{$\phi = \phi_1 \land \phi_2$}{
% \uIf{IsConjunctionTree($\phi_1$) $\land$ IsConjunctionTree($\phi_2$)}{
% \Return $\top$\;
% }
% \uElse{
% \Return $\bot$\;
% }
% }
% \uElseIf{$\phi = \mu$}{
% \Return $\top$\;
% }
% \uElse{
% \Return $\bot$\;
% }
% \end{algorithm}

% \begin{algorithm}
% \caption{ReachSample($\mathcal{R},t$)}
% \label{alg:sample}
% \uIf{Unif$(0,1) < 0.05$ \ri{define the goal bias explicitly later}}{
% \For{$R \in \mathcal{R}$}{
% \If{$t < t_1 \lor t > t_2$}{
% $\mathcal{R} = \mathcal{R} \symbol{92} R$\;
% }
% }
% $R_{sample} =$ Unif($\mathcal{R}$)\;
% $s_{sample} = $ Unif($x \in X | x \vDash R_{sample}$)\;
% }
% \uElse{
% $s_{sample} = $ Unif($x \in X)$\;
% }
% \end{algorithm}
% \ri{try to make all functions either italicized or regular, not both}

==> ICRA23_sections/StoRI.tex <==
\section{Stochastic Robustness Measure}
\label{sec:stori}

% \ml{DEFINED MACROs $\backslash low\{ \}$ and $\backslash up\{ \}$ for lower and upper bounds as underline and bar, respectively. USE THEM!}

\iffalse
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
     Experiment & Success Rate & average computation time (s) \\
     \hline
     Until, \stori 0.5 & 91\% & 82.98 $\pm$ 79.67 \\
     Until, \stori 0.8 & 80\% & 71.9 $\pm$ 64.45 \\
     not Until, \stori 0.5 & 89\% & 73.59 $\pm$ 76.79 \\
     not Until, \stori 0.8 & 90\% & 70.14 $\pm$ 64.49 \\
     \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
\fi

A popular method of measuring robustness of belief trajectories in motion planning is based on the notion of chance constraints \cite{blackmore2006probabilistic,luders2010chance,ho2022gaussian}. Chance constraints require that the probability of constraint violation (e.g., avoiding obstacles) not exceed some prescribed value. Motion planners typically enforce this chance constraint at each time step. 

Such an approach is difficult to extend to STL formulas. This is primarily due to temporal operators and their time intervals,
e.g., the probability of violating $\Diamond_I \phi$ only needs to be below a prescribed value at one time step in $I$, but it is not clear at which time step to enforce this. 
Some approaches find success by generating constraints over time windows, and allocating risk of violating the constraints among time steps~\cite{C2TL,farahani2018shrinking}. However, those methods are limited to reasoning about discrete-time trajectories. This is in conflict with the fundamental idea of STL, which is expressing properties over real-valued continuous-time intervals.

Furthermore, those approaches only provide a \textit{qualitative} (boolean) judgement of a trajectory's satisfaction with respect to a chance constraint. In contrast, we seek to define a measure that provides a \textit{quantitative} judgement of a trajectory's satisfaction. This is analogous to robustness for deterministic STL that provides a quantitative measure beyond the qualitative Boolean semantics. Such a measure can then be extended to reason about partial trajectories, and hence, is advantageous for iterative methods for planning such as sampling-based algorithms. To illustrate what such a measure might convey, consider the following example.
\begin{example}
    \label{ex:intuition}
    \emph{
    Consider the formulas $\phi_1 = \square_I \mu$ and $\phi_2 = \Diamond_I \mu$. In the case of the $\square$ operator, which states that a property must hold for all time $ t \in I$, a quantitative measure of robustness
    could be characterized by the point with the lowest probability of satisfying $\mu$ in $I$, i.e., $\min_{t\in I} P(h(\xtraj(t)) \geq 0)$, where $h$ is the linear function that $\mu$ is defined on. If the probability of violation at that point is below a certain threshold, then it is also below that threshold at every other point. Similarly, for the $\Diamond$ operator, which states that a property must hold for \textit{a} time point $ t \in I$, we could look at the point with the \textit{highest} probability of satisfying $\mu$, i.e., $\max_{t\in\langle a,b \rangle} P(h(\xtraj(t)) \geq 0)$. If the probability of violation at that point is above a certain threshold, then formula $\phi_2$ is satisfied. A quantitative measure of stochastic robustness must incorporate this conflicting treatment of 
    temporal operators.
    }
\end{example}
This intuition guides the development of the Stochastic Robustness Interval (\stori) as defined below. 


% Consider the formula $\phi_1 = \square_{[0,10]}\lnot (\mu_1 \land \mu_2)$, which states that, for every time point between $t=0$ and $t=10$, avoid the region defined by predicates $\mu_1$ and $\mu_2$. We are interested in quantifying and constraining the point in the trajectory $\btraj$ with the highest probability of occupying the region. If this point satisfies a given constraint, then every other point also satisfies the constraint and the trajectory satisfies $\phi_1$.  

% In contrast, consider the formula $\phi_2 = \Diamond_{[0,10]} (\mu_1 \land \mu_2)$ (at any point between $t=0$ and $t=10$, reach region the region defined by predicates $\mu_1$ and $\mu_2$). We are interested in quantifying and constraining the point in the trajectory $\btraj$ with the highest probability of occupying the region. If any point satisfies a given constraint, then the trajectory is satisfies $\phi_2$. 
% For both of these formulas, we are interested in complete trajectories that are defined at all points in time in the formulas
% \ml{this sentence is unclear}
% . 

% % \qh{Don't use contractions in technical writing, see page 21 of \url{http://journals.ieeeauthorcenter.ieee.org/wp-content/uploads/sites/7/IEEE-Editorial-Style-Manual-for-Authors.pdf}}

% \ml{the following paragraph is unclear... want to say that the measure must reason over the probability bounds over linear predicates. That is because ...???}
% Furthermore, because STL is defined over predicates, we would  like to work with upper and lower bounds for the probabilities of occupying regions
% \ml{need to explain why we care about the bounds!} \ri{I feel like i do? right below this}, calculated from the probabilities of satisfying the linear predicates that define the regions. Both the upper and lower bounds are necessary; We would like to constrain the upper bound in $\phi_1$ above, but constrain the lower bound in $\phi_2$ above. This intuition guides the development of the Stochastic Robustness Interval (\stori) as defined below. 


% \ml{once active predicates is defined, then we can define the measure as follows.\\
% Given trajectory $x$, let $P(x, t, \phi)$ be the probability that point $x(t)$ on the trajectory satisfies the active predicates at time $t$. Then, the measure is defined as:
% $$f(\phi,x) = \min_{t} P(x, t, \phi)$$
% }

% \subsection{Definition}
\begin{definition}[Stochastic Robustness Interval]
    \label{def:stori}
    The Stochastic Robustness Interval (\stori) of a belief trajectory $\btraj$ over time window $[0,T]$ with respect to an STL formula $\phi$ is a functional $f(\phi, \btraj)$:
    \begin{equation*}
        f(\phi, \btraj) = [\low{f}(\phi, \btraj), \up{f}(\phi,  \btraj)]
    \end{equation*}
    such that $0 \leq \low{f}(\phi,\btraj) \leq \up{f} (\phi,\btraj) \leq 1$.  
    For a $t \in [0,T]$,
    let $\btraj^t$ be the time-shifted suffix of trajectory $\btraj$ such that %$\btraj^t(0) = \btraj(t)$ and, 
    for all $t' \in [0,T-t]$, $\btraj^t(t') = \btraj(t+t')$. 
    Then, lower bound $\low{f}(\phi,\btraj)$ and upper bound $\up{f}(\phi,\btraj)$ are recursively defined by:
    % \begin{align*}
    %     &\low{f}(\top,\btraj) &&= 1 \\
    %     &\low{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\low{f}(\lnot \phi, \btraj) &&= 1 - \up{f}(\phi,\btraj) \\
    %     &\low{f}(\phi_1 \land \phi_2, \btraj, t) &&= \max\big\{\low{f}(\phi_1,\btraj) + \low{f}(\phi_2,\btraj) -1,0\big\} \\
    %     &\low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=   
    %     \Big\{ \displaystyle \max_{t\in\langle a,b \rangle} \big\{ \max \{\low{f}(\phi_2,\btraj^t) \\
    %     & && \qquad \qquad + \min_{t'\in[0,t]}\low{f}(\phi_1,\btraj^{t'}) \} - 1,0 \big\} \Big\} 
    % \end{align*}
    % \begin{align*}
    %     &\up{f}(\top, \btraj) &&= 1 \\
    %     &\up{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\up{f}(\lnot \phi, \btraj) &&= 1 - \low{f}(\phi,\btraj) \\
    %     &\up{f}(\phi_1 \land \phi_2, \btraj, t) &&= \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\} \\
    %     &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=  \\ 
    %     \rlap{$\displaystyle \max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\} \Big\} $} \\
    % \end{align*}
    \begin{align*}
        &\low{f}(\top,\btraj) = \up{f}(\top, \btraj) = 1, \\
        &\low{f}(\mu, \btraj) = \up{f}(\mu, \btraj) = P(h(x(0)) \geq 0 ), \\
        &\low{f}(\lnot \phi, \btraj) = 1 - \up{f}(\phi,\btraj), \\
        &\up{f}(\lnot \phi, \btraj) = 1 - \low{f}(\phi,\btraj), \\
        \end{align*} 
        \begin{align*}
        &\low{f}(\phi_1 \land \phi_2, \btraj) = \max\big\{\low{f}(\phi_1,\btraj) + \low{f}(\phi_2,\btraj) -1,0\big\}, \\
        &\up{f}(\phi_1 \land \phi_2, \btraj) = \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\}, \\
        &\low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = \\
        & \quad \max_{t\in\langle a,b \rangle} \Big\{ \max \big\{\low{f}(\phi_2,\btraj^t) + \min_{t'\in[0,t]}\low{f}(\phi_1,\btraj^{t'}) - 1,0\big\} \Big\}, \\
        &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = \\
        & \quad \max_{t\in\langle a,b \rangle} \Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\}\Big\}.
    \end{align*}
    % \begin{align*}
    %     &\up{f}(\top, \btraj) &&= 1 \\
    %     &\up{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\up{f}(\lnot \phi, \btraj) &&= 1 - \low{f}(\phi,\btraj) \\
    %     &\up{f}(\phi_1 \land \phi_2, \btraj, t) &&= \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\} \\
    %     &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=  \\ 
    %     \rlap{$\displaystyle \max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\} \Big\} $} \\
    % \end{align*}
\end{definition}



We define the Stochastic Robustness Measure (\storm) to be the lower bound of \stori. 


\begin{definition}[Stochastic Robustness Measure]
    \label{def:StochRo}
    The \emph{Stochastic Robustness Measure} (\storm) of a belief trajectory $\btraj$ with respect to STL formula $\phi$ is the lower bound of the \stori, i.e, $\low{f}(\phi, \btraj)$.
\end{definition}

The \stori is an interval that aims to quantify how robustly a belief trajectory $\btraj$ satisfies an STL formula $\phi$. The \storm of a belief trajectory is the lower bound of its \stori. 
A trajectory always satisfies a Boolean $\top$, so the \stori for $\phi = \top$ is $[1,1]$ for every trajectory. If $\phi = \mu$ is a linear predicate, both bounds of the \stori are the probability that the state at time zero $x(0)$
% \ml{this is not right... $\hat{x}(0)$ is not a random variable so the probability is either 0 or 1.}\ri{it applies to the time shifted trajectories; b(0) of the t-shifted suffix trajectory is a distribution (like think of how we check globally - shift it for every t and look at the first "0th" element)}
satisfies the linear predicate. Works \cite{blackmore2006probabilistic} \cite{pairet2021} outline an efficient way to calculate this probability for Gaussian distributions. However, we stress that the \stori is defined for general belief distributions, and also applies to non-Gaussian beliefs. 

The \stori of the negation of a formula $\lnot \phi$ derives from the Unit Measure Axiom of Probability \cite{ProbBook}. Note that the lower bound of the \stori of $\lnot\phi$ depends on the upper bound of the \stori of $\phi$, and vice-versa. 


\begin{figure*}
\centering
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/certain.eps}
  \hfill
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/uncertain.eps}
  \hfill
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/fast_example.eps}
\caption{Sample trajectories that have a \stori of (left-to-right) $[0.72, 0.91]$, $[0.52, 0.847]$, $[0, 0]$ with respect to $\varphi_1$ in \eqref{eq:form1}}
\label{fig:examples}
\end{figure*}

The \stori for a conjunction of two formulas $\phi_1 \land \phi_2$ is inspired by the lower and upper bounds on the probability of a conjunction of two events. These are the Boole-Fr\'echet inequalities for logical conjunction \cite{frechet1935generalisation}, which make no assumptions on the independence on the events, and hence are general. Note that the measure seeks to quantify both upper and lower bounds because the upper bound is conservative when the specification seeks to enforce `avoidance' of the conjunction, but the lower bound is conservative when it seeks to enforce the `occupancy' of the conjunction. 

% The \stori for a conjunction of two formulas $\phi_1 \land \phi_2$ is inspired by the lower and upper bounds on the probability of a conjunction of two events; For any set of probabilistic events ${h_i}$, the probability of their conjunction is bounded by:
% \ri{if we keep this, should I use this general form for the equation or the simplified form for two events?}\qh{Write general form for now}
% \begin{equation}
%     \left(\sum_{i=1}^n P(h_i)\right) - n + 1 \leq P(\land_{i=1}^n h_i) \leq \min_i P(h_i)
% \end{equation}

% Because of this, the \stori of a conjunction of two predicates $f(\mu_1 \land \mu_2,\hat{\btraj})$ exactly bounds the probability that the belief at time zero satisfies both predicates $P(\hat{x}(0) \vDash \mu_1 \land \hat{x}(0) \vDash \mu_2)$. Furthermore, it provides useful quantitative information on the stochastic robustness of a trajectory when considering the conjunction of multiple formulas $f(\phi_1 \land \phi_2,\hat{\btraj})$. The \stori of a negation of a formula $\lnot \phi$ similarly derives from probability theory. 

% \ml{do we need this?  it's obvious... and also we don't have room for it}
% Logical disjunction of two formulas $\phi_1 \lor \phi_2 = \lnot (\lnot \phi_1 \land \lnot \phi_2)$. Applying the \stori to this form correctly results in the Boole-Fr\'echet inequalities for logican disjunction, i.e.,
% % \begin{equation}
% \begin{align}
%     \low{f}(\phi_1 \lor \phi_2) &= \max\big\{\low{f}(\phi_1,\btraj), \low{f}(\phi_2,\btraj)\}, \\
%     \up{f}(\phi_1 \lor \phi_2) &= \min\big\{\up{f}(\phi_1,\btraj) + \up{f}(\phi_2,\btraj),1\big\}.
% \end{align}
% % \end{equation}







The \stori of $\phi_1 U_{\langle a,b \rangle} \phi_2$ is less straightforward. Intuitively, it aims to report the 
% Stochastic Robustness Measure 
\storm
at the time $t \in \langle a,b \rangle$ that best balances the point-wise probabilities that $\phi_1$ hold for all $t' \in [0,t]$ and the probability that $\phi_2$ hold at $t$. 

Note that by following Definition \ref{def:stori}, the obtained \stori for eventually and globally are: 
\begin{align}
    f(\Diamond_{\langle a,b\rangle} \phi, \btraj) &= \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\btraj^t), \; \max_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg] 
\end{align}
\begin{align}
    f(\square_{\langle a,b\rangle} \phi, \btraj) &= \bigg[\min_{t \in \langle a, b\rangle} \low{f}(\phi,\btraj^t), \; \min_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg]  
\end{align}

\noindent
These intervals are fully inline with the intuition of the measure as discussed in Example~\ref{ex:intuition}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD DERIVATION (LOOKS NICE MAYBE ARXIV VERSION?
% The \stori of the temporal operator $eventually$, traditionally defined as $\Diamond_{[a,b]}\phi = \top U_{[a,b]} \phi$, is derived by considering that $f(\btraj,\top) = [1,1]$:

% \begin{align*}
%         &\low{f}(\top U_{\langle a,b \rangle} \phi, \btraj) \\ 
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \max \big\{\low{f}(\phi,\btraj^t) + \min_{t'\in[0,t]}\low{f}(\top,\btraj^{t'}) - 1,0 \big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \max \big\{\low{f}(\phi,\btraj^t) + 1 - 1,0 \big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\big\{ \low{f}(\phi,\btraj^t) \big\} \\
%         &\up{f}(\top U_{\langle a,b \rangle} \phi, \btraj)\\ 
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi,\btraj^t), \min_{t'\in[0,t]}\up{f}(\top,\btraj^{t'})\big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi,\btraj^t), 1\big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\big\{ \up{f}(\phi,\btraj^t) \big\} \\
%         &\Rightarrow f(\Diamond_{[a,b]} \phi, \btraj) = \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\btraj^t),\max_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg]  \\
% \end{align*}

% \ri{we can take out this derivation if you guys want, I feel like it's satisfying to show but we can either not show any, just show this, or I can also give quick derivations for globally and disjunction as well.}

% This agrees with the intuitively expected value presented at the beginning of this section. Similarly, the \stori of the temporal operator \textit{globally}, traditionally defined as $\square_{\langle a, b\rangle} \phi = \lnot \Diamond_{\langle a,b\rangle} \lnot \phi$, also agrees with the intuition: 

% \begin{equation*}
%     f(\square_{[a,b]} \phi, \btraj) = \bigg[\min_{t \in [a,b]} \low{f}(\phi,\btraj^t),\min_{t \in [a,b]} \up{f}(\phi,\btraj^t)\bigg]  
% \end{equation*}



% \subsection{Examples}
\begin{example}
    \label{ex:stori}
    \emph{
    % In this section, we present examples of the \stori as it relates to a couple sample trajectories. 
    Consider the environment in Fig. \ref{fig:examples} and formula
    \begin{equation}
    \label{eq:form1}
        \varphi_1 = \neg (x\geq 1 \wedge y \geq 2 \wedge x \leq 2) U_I (x \geq 3 \wedge y \geq 2).
    \end{equation}
    % which specifies that the robot must avoid the obstacle until it reaches the goal at some time $t \in I$. 
    Fig. \ref{fig:examples} shows three belief trajectories, where the ellipses represent the 90\% confidence bounds of their uncertainty. 
    The first two trajectories (left and middle) have the same expectation but are subject to different amounts of process noise. 
    When evaluating against $\varphi_1$ with time interval $I = [0,6]$,
    we see both bounds of the \stori decrease
    from $[0.72, 0.91]$ for the first trajectory (left) to $[0.52, 0.85]$ for the
    the second trajectory that has more uncertainty (middle). This trajectory is less likely to clear the obstacle, and also less likely to arrive in the goal region. The third plot (right) shows the first trajectory but evaluated against $\varphi_1$ with smaller interval $I = [0, 4]$. The robot does not arrive to goal until after 5 seconds. Hence, the robot fails to satisfy the specification and its \stori is $[0, 0]$.
    }
\end{example}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

An important property of the \stori is that a trajectory which has a \storm of 1 satisfies STL formula $\phi$ with probability 1, as stated in the following theorem, which illustrates soundness of \storm. 
% \ml{not sure about the following... should perhaps remove it.}
% \ri{In other words, the \storm is sound with respect to the semantics of STL.}

% \subsection{Soundness} 
% The soundness of our proposed stochastic robustness interval measure is stated formally in the following theorem.

\begin{theorem}
Given belief trajectory $\btraj$ and STL formula $\phi$, if the Stochastic Robustness Measure $\low{f}(\phi,\btraj) = 1$, then every realization $\xtraj$ of $\btraj$ satisfies the specification, i.e., $\xtraj \models \phi$, except realizations on the set of measure zero.
\end{theorem}
% \qh{Prove the converse for $\up{f}(\phi,\btraj) = 0$}
\begin{proof}[Proof Sketch]
     The proof follows the recursive definition of \stori, and the fact that $\low{f}(\phi,\btraj) \leq \up{f} (\phi,\btraj)$. If $\low{f}(\mu,\btraj) = 1$, this implies that $P(h(\xtraj(0)) \geq 0) = 1$, i.e., almost every realization of the trajectory satisfies the predicate $\mu$. Since $\phi$ is recursively defined by $\top$ and $\mu$, by the recursive definition of \stori, we see that $\low{f}(\phi, \btraj) = 1$ implies that almost every realization of the trajectory satisfies $\phi$. A detailed proof is provided in the extended version of this paper \cite{Ilyes2022extended}.
\end{proof}



% \begin{figure}[ht]
% \centering
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/certain_example.png}
%   \caption{}
%   \label{fig:ex1} 
% \end{subfigure}
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/uncertain_example.png}
%   \caption{}
%   \label{fig:ex2}
% \end{subfigure}
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/fast_example.png}
%   \caption{}
%   \label{fig:ex3}
% \end{subfigure}
% \caption{Sample Trajectories that have a \stori of (a) [0.72,0.91], (b) [0.524,0.847], (c) [0,0] with respect to $\phi_1$}
% \end{figure}

% \begin{figure}[ht]
% \centering
%   \includegraphics[width=\linewidth]{figures/certain_example.png} 
%   \\\vspace{-5mm}
%   \includegraphics[width=\linewidth]{figures/uncertain_example.png}
%   \\\vspace{-10mm}
%   \includegraphics[width=\linewidth]{figures/fast_example.png}
%   \\\vspace{-5mm}
% \caption{Sample Trajectories that have a \stori of (top-to-bottom) [0.72,0.91], [0.524,0.847], [0,0] with respect to $\phi_1$}
% \label{fig:examples}
% \end{figure}



% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/certain_example.png}
%     \caption{Trajectory for $\phi_1$ with a \stori of [0.72,0.91]}
%     \label{fig:ex1}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/uncertain_example.png}
%     \caption{Trajectory for $\phi_1$ with a \stori of [0.52,0.85]}
%     \label{fig:ex2}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/fast_example.png}
%     \caption{Trajectory for the modified $\phi_1$ with a \stori of [0,0]}
%     \label{fig:ex3}
% \end{figure}

\subsection{\stori Monitor}

% Trajectory prefixes, though not complete, still contain behavior relevant to the satisfaction of STL formulas. Partial trajectories may reveal if a safety property has been violated or a liveliness property has been satisfied. 

\stori is defined for a given belief trajectory. It does not account for \emph{what could happen if we extend the trajectory.}
However, in some cases (such as planning), we are interested in extending trajectories to achieve a higher \storm. Hence, we need a monitor for \stori, which assumes the given trajectory is to be extended. The monitor must account for all the possible suffixes of the trajectory and how they might change the \storm. In this section, we present a monitor for the \stori with respect to a partial belief trajectory, that acts to bound the achievable \stori of any extensions of it.

\begin{definition}[StoRI Monitor]
    \label{def:Monitor}
    The Stochastic Robustness Interval (\stori) Monitor of a partial belief trajectory $\ptraj$ over time window $[0,t]$ with respect to an STL formula $\phi$ is a functional $\Tilde{f}(\phi, \ptraj)$:
    \begin{equation*}
        \Tilde{f}(\phi, \ptraj) = [\low{\Tilde{f}}(\phi, \ptraj), \up{\Tilde{f}}(\phi, \ptraj)]
    \end{equation*}
    such that $0 \leq \low{\Tilde{f}}(\phi,\ptraj) \leq \up{\Tilde{f}} (\phi,\ptraj) \leq 1$,
    where
    \begin{align*}
        &\Tilde{f}(\top,\ptraj) = f(\top,\ptraj) \\
        &\Tilde{f}(\mu,\ptraj) = f(\mu,\ptraj) \\
        &\low{\Tilde{f}}(\lnot \phi, \ptraj) = 1 - \up{\Tilde{f}}(\phi,\ptraj), \\
        &\up{\Tilde{f}}(\lnot \phi, \ptraj) = 1 - \low{\Tilde{f}}(\phi,\ptraj), \\
        &\low{\Tilde{f}}(\phi_1 \land \phi_2, \ptraj, t) = \max\big\{\low{\Tilde{f}}(\phi_1,\ptraj) + \low{\Tilde{f}}(\phi_2,\ptraj) -1,0\big\}, \\
        &\up{\Tilde{f}}(\phi_1 \land \phi_2, \ptraj, t) = \min\big\{\up{\Tilde{f}}(\phi_1,\ptraj), \up{\Tilde{f}}(\phi_2,\ptraj)\}, \\
        &\low{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) = 
        \begin{cases}
             \low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) & \text{if } t \geq a \\ 
            0 &\text{otherwise,}
        \end{cases} \\
        &\up{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) = \\ 
        &
        \begin{cases}
            \up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj)
            & \hspace{-2mm} \text{if } t \geq b\\
            \displaystyle \max \hspace{-.5mm} \Big\{\hspace{-.5mm}\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj), \min_{t'\in[0,b]}\up{f}(\phi_1,\ptraj^{t'}) \hspace{-.5mm} \Big\} & \hspace{-2mm} \text{if } t \in [0,b) \\ 
            1 & \hspace{-2mm} \text{otherwise.}
        \end{cases}
    \end{align*}
    % \ml{the middle condition, shouldn't it be $t \in [a, b)$?}
\end{definition}
% \ri{double check: which case up top should include t = b? while we're at it, check all of the inequalities}\ri{OOF i actually feel like this depends on whether $I$ is a closed or open interval, right?? how do we do this nicely?}
% \ml{unclear}

The differences between the \stori and \stori Monitor arise in the temporal operators. These operators seek to bound possible future robustness, and also quantify the robustness of the behavior already seen. This is apparent in the \stori Monitor with respect to the $\Diamond$ and $\square$ operators:

% \ri{old/incorrect versions: }
% \begin{align}
%     \Tilde{f}(\Diamond_{\langle a,b \rangle} \phi, \ptraj) &= \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\ptraj^t), \;1\bigg]  \\
%     \Tilde{f}(\square_{\langle a,b \rangle } \phi, \ptraj) &= \bigg[0, \; \min_{t \in \langle a,b \rangle} \up{f}(\phi,\ptraj^t)\bigg]  
% \end{align}
% \ri{correct versions: }
\begin{align*}
    \Tilde{f}(\Diamond_{\langle a,b \rangle} \phi, \ptraj) =  
    &
    \begin{cases}
        f(\Diamond_{\langle a,b \rangle} \phi, \ptraj) &\text{if } t \geq b \\
        \Big[\max\limits_{t \in \langle a,b \rangle} \low{f}(\phi,\ptraj^t), \;1\Big]& \text{if } a \leq t < b \\
        \big[0,1\big]& \text{if } t < a
    \end{cases} \\
    \Tilde{f}(\square_{\langle a,b \rangle } \phi, \ptraj) = 
    &
    \begin{cases}
        f(\square_{\langle a,b \rangle } \phi, \ptraj) &\text{if } t \geq b \\
        \Big[0, \; \min\limits_{t \in \langle a,b \rangle} \up{f}(\phi,\ptraj^t)\Big]& \text{if } a \leq t < b \\
        \big[0,1\big]& \text{if } t < a
    \end{cases} 
\end{align*} 

The case when $a\leq t < b$ is of particular interest. In the case of the $\square$ operator, the \stori is upper bounded by the best point in the partial trajectory, but is lower bounded by zero to account for possible future violation. In the case of the $\Diamond$ operator, the \stori is lower bounded by the best point in the partial trajectory, but is upper bounded by one to account for possible future ``perfect" satisfaction. 

The following theorem proves the correctness of \stori Monitor by showing that it always subsumes \stori.

\begin{theorem}
    \label{theorem:monitorbounds}
    Let $\btraj$ be a belief trajectory over time window $[0,T]$ and $\btraj_t$ be a prefix of $\btraj$ where $t \in [0,T]$.  Then, given STL formula $\phi$, the StoRI Monitor for $\btraj_t$ subsumes the StoRI of $\btraj$ for all $t \in [0,T]$, i.e., $\forall t \in [0,T]$, $f(\phi,\btraj) \subseteq \Tilde{f}(\phi,\btraj_t)$.
\end{theorem}
\begin{proof}[Proof Sketch]
    Due to space constraints, we provide the general sketch of this proof. A detailed proof is provided in the extended version of this paper \cite{Ilyes2022extended}. Without loss of generality, consider $\phi = \psi_1 U_{[a,b]} \psi_2$. Using definitions \ref{def:Monitor} and \ref{def:stori}, the main idea of the proof comes from the fact that the upper bound is a monotonically decreasing function, and that the lower bound is a monotonically increasing function. Additionally, for a complete trajectory $\btraj$, $\up{\Tilde{f}}(\phi,\btraj) \geq \up{f}(\phi,\btraj)$ and $\low{\Tilde{f}}(\phi,\btraj) \leq \low{f}(\phi,\btraj)$.
\end{proof}

% From definition \ref{def:Monitor}, we see that the upper bound of the \stori Monitor $\up{\Tilde{f}}(\phi,\ptraj) \geq \up{f}(\phi,\btraj)$. Similarly, the lower bound of the \stori Monitor $\low{\Tilde{f}}(\phi,\ptraj) \leq \low{f}(\phi,\btraj)$. Therefore, $f(\phi,\btraj) \subseteq \Tilde{f}(\phi,\btraj_t)$. \ri{is it that simple? feel like this isn't right}. 

\begin{example}
    \label{ex:monitor}
    \emph{
    Recall the STL formula in Example~\ref{ex:stori} and sample trajectories in Fig. \ref{fig:examples}.
    The \stori Monitor of the trajectories at different points in their evolution are shown in the plots in Fig. \ref{fig:examples}. Note that they subsume the \stori of the final trajectory and the interval gets smaller with time. 
    }
\end{example}

==> sections/Conclusion.tex <==
\section{Conclusion and Future Work}
This paper proposes a measure, \storm, for quantifying the robustness of stochastic systems' trajectories with respect to STL specifications. We develop a monitor for this measure that reasons about partial trajectories, and use it in a sampling-based motion planner. We show desirable properties of this measure, that the algorithm is probabilistically complete, and that the algorithm asymptotically optimizes for the \storm. Emprical evaluation demonstrates the measure and algorithm's effectiveness and utility. For future work, we plan to investigate methods to guide the growth of the motion tree and incorporate measurement uncertainty in the motion planner. \ri{to-do: mention investigating how this ties to probability of satisfaction in future work}

==> sections/Experiments.tex <==
\section{Evaluations}
We evaluate efficacy and efficiency of the proposed measure and planners subject to a variety of STL specifications. The algorithms are implemented with \X= RRT \cite{RRT}, i.e., \stori-RRT. All algorithms are implemented in the Open Motion Planning Library (OMPL)~\cite{sucan2012the-open-motion-planning-library}, and computations were performed on 3.9 GHz CPU and 64 GB of RAM. 

We considered a noisy second-order unicycle system whose stochastic dynamics are given by:
% \begin{equation}
% \label{eq:unicycle}
    $dx = v \cos(\theta) dt + dw$, 
    $dy = v \sin(\theta) dt + dw$,
    $d\theta = u_\omega dt + dw$,
    $dv = u_a dt + dw$
% \end{equation}
where $u_a$ and $u_\omega$ are the acceleration and steering angle inputs. We linearized the dynamics according to the feedback linearization in \cite{unicycle}.  We considered environments in Figs. \ref{fig:examples}, \ref{fig:form2}, and \ref{fig:form4} respectively  with STL formulae $\varphi_1$ in \eqref{eq:form1}, 
\begin{align}
    \varphi_2 &= \lnot O U_{[0,10]} A \land \lnot O U_{[0,10]} B, \label{eq:form2}\\
    % &W = x \geq 0 \land x \leq 4 \land y \geq -2 \land y \leq 2 \notag\\
    &O = x \geq 1.5 \land x \leq 3.5 \land y \geq -0.5 \land y \leq 0.5, \notag\\
    &A = x \geq 2 \land x \leq 3 \land y \geq 1, \notag\\
    &B = x \geq 2 \land x \leq 3 \land y \leq -1, \notag\\
    \varphi_3 &= (\text{Puddle} \rightarrow \lnot \text{Charge} U_{[0,3]} \text{Carpet}) U _{[0,10]} \text{Charge}, \label{formeq:3}\\
    &\text{Puddle} = y \leq 2.5 \land x \geq 2 \land x \leq 3, \notag\\
    &\text{Charge} = y \geq 2 \land x \geq 4, \notag\\
    &\text{Carpet} = y \leq 1 \land x \geq 4. \notag
\end{align}
% $\text{Charge} = y \geq 2 \land x \geq 4$, and $\text{Carpet} = y \leq 1 \land x \geq 4$.
Here, $\varphi_2$ requires avoiding (black) region $O$ until both regions $A$ and $B$ are visited within 10 minutes in Fig. \ref{fig:form2}. $\varphi_3$ requires the robot to go to the charger within 10 minutes and also that, if it visits the puddle, it must avoid the charger until it visits the carpet within 3 minutes of visiting the puddle in Fig. \ref{fig:form4}. For all formulas, we also enforce that the robot remains in their respective workspaces for the duration of the mission. 

\subsection{Case Study 1 - Computation Time vs \stori Threshold}

This case study seeks to analyze the relationship between computation time and the \storm constraint $\kappa$. Specifically, we study how \stori-RRT performs 
% when planning motions for system \ref{eq:unicycle} subject to STL 
for formula $\varphi_2$, in the environment in Fig. \ref{fig:form2}. 
We ran $100$ trials, with a maximum computation time of $300$ seconds for each trial. 
Table \ref{tab:bench1} reports the computation time and success rate for different $\kappa$ values. We see that computation time increases and success rate decreases as the $\kappa$ threshold increases. This is due to the increased difficulty of satisfying the robustness constraint.

\begin{table}[h]
    \centering
    \caption{Benchmarking Results for Case Study 1}
    \begin{tabular}{|c|c|c|}
    \hline
        \storm Threshold $\kappa$ & Computation Time (s) & Success Rate\\ 
        \hline
        0.5 & 60.10 $\pm$ 64.87 & 97\%\\
        0.7 & 71.37 $\pm$ 67.48 & 97\%\\
        0.9 & 83.30 $\pm$ 69.35 & 90\%\\
        0.95 & 92.48 $\pm$ 81.56 & 86\%\\
        \hline
    \end{tabular}
    \label{tab:bench1}
    % \vspace{-3mm}
\end{table}

Fig. \ref{fig:form2} shows two sample trajectories for this specification, where the ellipses represent the 90\% confidence
bounds of their uncertainty. Trajectory 1 uses $\kappa = 0.9$ and goes through the wider opening on the left. In contrast, Trajectory 2 uses $\kappa = 0.5$ and finds less robust paths that go through the narrow opening on the right. 

\begin{figure}[t]
\centering
\begin{subfigure}{0.235\textwidth}
    \centering
    \includegraphics[width=\linewidth,trim={1cm 0cm 2cm 0cm},clip]{figures/form2.eps}
    \caption{$\phi_2$ Trajectories}
    % \caption{Two Trajectories for formula $\phi_2$. Trajectory 1 has a \stori of [0.944,0.991] and trajectory 2 has a \stori of [0.78,0.781]}
    \label{fig:form2}
\end{subfigure}
\begin{subfigure}{0.235\textwidth}
    \centering
    \includegraphics[width = \linewidth,trim={1cm 0 2cm 0},clip]{figures/bench3.eps}
    \caption{Case Study 3 Benchmark}
    \label{fig:case3}
\end{subfigure}
\caption{Experiment Results. (a) shows two trajectories where $\low{f}(\varphi_2,\btraj_1) = 0.98, \low{f}(\varphi_2,\btraj_2) = 0.67$, and (b) shows benchmarking results for Case Study 3}
\label{fig:results}
% \vspace{-3mm}
\end{figure}



\subsection{Case Study 2 - Computation Time for Different Formulas}
This case study compares computation time for different STL formulas. Table \ref{tab:bench2} shows the average computation time of \stori-RRT for the three formulas and environments over 100 trials with a maximum timeout of 300s. We used \storm bound $\kappa = 0.9$. We see that, even with a tight \storm threshold $\kappa$, the algorithm finds solutions with a good success rate and computation time. This shows that the algorithm is generally applicable to all STL formulas. 

\begin{table}[t]
    \caption{Benchmarking Results for Case Study 2, $\kappa = 0.9$.}
    \label{tab:bench2}
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
        Formula & Computation Time (s) & Success Rate\\ 
        \hline
        $\varphi_1$ & 1.98 $\pm$ 2.56 & 100\%\\
        $\varphi_2$ & 85.95 $\pm$ 82.56 & 90\%\\
        $\varphi_3$ & 44.55 $\pm$ 53.89 & 99\%\\
        \hline
    \end{tabular}
    %  \vspace{-3mm}
\end{table}

\subsection{Case Study 3 - Asymptotic Optimality}
In this case study, we analyze the relationship between given computation time and the \storm of the resulting trajectory. Here, we study how AO-\stori-RRT performs when planning for formula $\varphi_3$, in the environment in Fig. \ref{fig:form4}. Fig. \ref{fig:case3} presents the results of 100 trials. It clearly shows that the solutions asymptotically approach an optimal \storm. Fig. \ref{fig:form4} gives two sample trajectories with different {\storm}s. Trajectory 2 is found earlier in the optimization, and makes it through the gap. When the planner further optimizes for the \storm, however, it favors trajectories like Trajectory 1, that enter the puddle and dry off before going to the carpet. 



\subsection{Case Study 4 - Simulated Performance}
This case study seeks to analyze how the \storm relates to the statistical satisfaction rate. We do this by simulating the robot's motion plans from \stori-RRT. Table \ref{tab:corr} compares the \stori of the belief trajectories against the statistical satisfaction rate of the simulated realizations. Each motion plan is simulated 1000 times. We use the Breach Toolbox \cite{rosi} to evaluate the realizations' satisfaction. The results show that there is positive correlation between the \storm and the simulated rate of success.

\begin{table}[ht]
    \caption{Comparison of StoRI and statistical satisfcation rate for controllers synthesized with StoRI-RRT
    }
    \label{tab:corr}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        Formula & \storm & $\up{f}(\phi,\btraj)$ & Satisfaction Rate\\
        \hline
        $\varphi_1$ & 0.568 & 0.568  & 0.367\\
        $\varphi_1$ & 0.755 & 0.781  & 0.767\\
        $\varphi_1$ & 0.986 & 0.986  & 0.985\\ 
        \hline
        $\varphi_2$ & 0.572 & 0.589  & 0.582\\
        $\varphi_2$ & 0.873 & 0.998  & 0.754\\
        $\varphi_2$ & 0.912 & 0.913  & 0.889\\
        \hline
        $\varphi_3$ & 0.625 & 0.677  & 0.669\\ 
        $\varphi_3$ & 0.876 & 0.878  & 0.872\\
        $\varphi_3$ & 0.989 & 0.994  & 0.985\\
        \hline
    \end{tabular}
     \vspace{-3mm}
\end{table}
\ri{to-do: add note that \storm is $\low{f}(\phi,\btraj)$}
\ri{to-do: mention we empircally show correlation between StoRM and Prob of satisfaction}
\ri{to-do: define statistical satisfaction rate}



==> sections/Introduction.tex <==
\section{Introduction}
\label{sec:intro}

\qh{Make sure that StoRI and StoRI-Extended are edited the same}

\ri{to-do: better lit review}
\ri{clarify "proper" measure and why none of the existing works provide such a measure}
\ri{to-do: references -> 16 -> provide chapter number}
\ri{to-do: make sure our usage of set notation is correct and consistent}
\ri{to-do: motivate sampling based planners, mention the StoRI can be used in various frameworks but we developed it with sampling based planners in mind}
%P1 - introduce STL, Uncertainty, and Goal
In recent years, \emph{Temporal Logics} (TLs) \cite{Lahijanian:AR-CRAS:2017}
have been increasingly employed to formalize complex robotic tasks.  These logics allow precise description of properties over time by combining Boolean logic with temporal operators.  
% a wide variety of robotic tasks. 
A popular choice is \emph{Linear TL} \cite{BaierBook2008}, where time is treated as linear and discrete.  
However, robotic systems operate in continuous time, and their tasks often include properties in dense time. Signal TL (STL) \cite{Maler2004} is a variant of TL that  
provides the means for expressing such tasks with evaluations over continuous signals (trajectories).  
% What makes STL powerful, i.e., reasoning over continuous time, however,  
For motion planning, however, STL introduces both computational and algorithmic challenges precisely due to same reason that makes it powerful, i.e., reasoning in continuous time.  
% In deployment, these robots must also face uncertainty in their motion. Motion planning with STL is difficult, however, and the additional compexity that arises from uncertainty makes it even more so. 
This challenge is exacerbated in real-world robotics, where uncertainty cannot be avoided.  Hence, 
% In order to plan trustworthy motions, motion planners need a way of reasoning about the robustness of plans by accounting for uncertainty. This paper focuses on this need and aims to develop a robustness metric and use it in a motion planning algorithm.
motion planners must reason about the robustness of plans by accounting for uncertainty. This requires a proper notion of a robustness measure.  STL does in fact admit such a measure but only for deterministic trajectories \cite{donze2010robust}. No such a measure is known for stochastic systems.  
This paper takes on this challenge and aims to develop a stochastic robustness measure for STL with the purpose of using it for efficient motion planning with robustness guarantees.

%P2 - example figure
Consider the following mission for the robot in Fig. \ref{fig:form4}: \textit{
Go to the charger in the next 10 minutes. But, if you traverse a puddle of water, stay away from the charger until you dry off on the carpet within 3 minutes}. 
% \ri{minutes?? not seconds?}
Such a specification is easily captured in STL. 
% STL is an extension of Linear Temporal Logic (LTL) with real-time and real-valued constraints. 
Two sample trajectories of an uncertain robot are shown in Fig. \ref{fig:form4}, where the ellipses represent the 90\% confidence contours around the nominal trajectories. Here, both trajectories appear to satisfy the temporal aspects of the specification. However, their spatial robustness is different with regards to their uncertainty. Note that, even though the nominal component of Trajectory 2 gets to the charger without passing through the water puddle, its uncertainty ellipses overlap with the puddle and walls, making the it less robust than Trajectory 1 with respect to the task. A capable motion planner must be able to reason about the robustness of these trajectories with respect to both temporal and spatial aspects of the STL task algorithmically.
% \ri{not sure how much/little i should say about the figure here}. 

%P3 - review of (deterministic) STL approaches
Much of the literature for control synthesis for STL specifications have been focused on deterministic systems. Success has been found using optimization-based techniques \cite{raman2014,raman2015reactive,OPTSTL1,OPTSTL2}, control barrier function approaches \cite{CBFSTL}, and sampling-based methods \cite{vasile2017sampling,CDCPaper}. 
The sampling-based approaches are particularly suitable for robotics applications given their efficiency and scalability.
None of those methods, however, accounts for stochasticity in the robot's dynamics. 

% \ri{I think farahani describes traditional robustness as "disturbances coming from a bounded polytope," and we can maybe use that and say those approaches don't account for the disturbances being drawn from a known distribution}. 

\begin{figure}[t]
    \centering
    \includegraphics[width = .85\linewidth,trim={1.8cm 1.5 1.8cm 1.5},clip]{figures/form4.eps}
    \caption{Two Trajectories for $\varphi_3$ \qh{Reference the equation for $\varphi_3$ or write it here. I took a long time to find it}. Trajectory 1 has a \storm of 0.96 and Trajectory 2 has a \storm of 0.71}
    \label{fig:form4}
    \vspace{-2mm}
\end{figure}
%P4 - review of (stochastic) STL approaches and shortcomings
For systems under uncertainty with STL specifications, recent works propose methods for chance-constrained optimization \cite{C2TL, farahani2018shrinking, PrSTLBelta, PrSTLSadigh}. Work \cite{C2TL} specifically first defines a new logic based on STL, called Chance-Constrained TL (C2TL), and then synthesizes optimal controllers for C2TL specifications for systems with perception uncertainty. Work \cite{farahani2018shrinking} reasons about the probability of obtaining a positive deterministic robustness to synthesize controllers for discrete-time systems in a chance-constrained formulation. However, all of these approaches require discrete-time trajectories and they do not quantify the robustness of stochastic trajectories.

% \ml{not clear why one should care about motion planning with sampling-based methods....  Need to motivate it somewhere before the next paragraph.}

%P5 - preview of this paper
In this work, we develop a novel measure of the robustness of continuous-time stochastic trajectories with respect to STL specifications.  We refer to it simply as the \textit{Stochastic Robustness Measure} (\storm). \storm allows us to quantify how well a stochastic trajectory satisfies a specification. 
The measure is based on the recursive evaluation of the \textit{Stochastic Robustness Interval} (StoRI) according to the semantics of STL over continuous belief trajectories and the probability measure. We also propose a technique to compute the StoRI of partial trajectories, which allows us to reason about (monitor) the satisfaction robustness of the STL properties on an evolving belief trajectory.  
Next, we present a sampling-based algorithm that produces motion plans that can (i) satisfy a user-defined bound on \storm, or (ii) asympotically optimize for \storm. We prove the theoretical properties of the algorithm under \storm constraints, and demonstrate the effectiveness of our measure and planner on a variety of STL formulas in several case studies and benchmarks.

%P6 - explicitly state contributions
In summary, the contributions of this work are four-fold: (i) a novel measure (\storm) to quantify the robustness of stochastic trajectories against STL specifications, (ii) a new monitor to compute the robustness of partial trajectories, (iii) a probabilistically-complete planning algorithm that satisfies STL specifications with \storm constraints for systems under uncertainty and asymptotically optimizes for \storm, and (iv) a series of case studies and benchmarks that reveal properties of \storm and performance of the planner.
% \qh{somewhere we should say we prove the theoretical parts, soundness,correctness, etc}\ri{here in contributions or one paragraph up, in the summary?}
% \ml{maybe both!}
% \ri{ok well first we have to actually prove it}




==> sections/Methodology.tex <==
\section{Motion Planning Algorithm}
\label{sec:motion-planning}
This section presents two sampling-based motion planners that utilize \stori and the \stori Monitor. The first planner finds solutions that satisfy a given \storm constraint, and the second finds solutions that directly optimizes for the \storm. 

\subsection{StoRI-\X}
A kinodynamic sampling-based tree planner \X grows a motion tree in the state space $X$ according to the robot dynamics through sampling and extension procedures. 
We generalize planner \X to \stori-\X to generate plans for System~\eqref{eq:SDE} that are guaranteed to satisfy a given lower bound $\kappa$ on \storm with respect to STL formula $\phi$.  \stori-\X planner is outline in Alg. \ref{alg:StoRIX}.
\ri{to-do: clearly introduc $N$ and $\kappa$}
\ri{to-do: think of different letter since X is already used for state space}
\ri{arxiv version -> provide the algo's hyperparameters used in experimentation (Q,G,etc). final version -> mention they're in the arxiv version}

\begin{algorithm}
\caption{\stori-\X($X,U,\phi,\hat{x}_0,N,\kappa)$)}
\label{alg:StoRIX}
$P_0 \gets 0^{n \times n}$\;
$\mathbb{V} \gets \{(\hat{x}_0,P_0)\},\mathbb{E} \gets \emptyset $\;
$\mathbb{G} \gets \{\mathbb{V},\mathbb{E}\}$\;
\For{N iterations}{
    $\hat{x}_{rand},t_{rand},\hat{x}_{near},P_{near} \gets sample(X,\mathbb{V},T)$\;
    $\hat{x}_{new},P_{new} \gets $ Extend($\hat{x}_{near},P_{near},U$)\;
    \If{$\up{\Tilde{f}}(\phi,(\hat{x}_0,P_0)...(\hat{x}_{new},P_{new})) > \kappa$}{
        $\mathbb{V} \gets \mathbb{V} \cup \{(\hat{x}_{new},P_{new})\}$ \;
        $\mathbb{E} \gets \mathbb{E} \cup \{[(\hat{x}_{near},P_{near}),(\hat{x}_{new},P_{new})]\}$\;
        \If{$\low{f}(\phi,(\hat{x}_0,P_0)...(\hat{x}_{new},P_{new})) > \kappa$}{
            \Return $(\hat{x}_0,P_0)...(\hat{x}_{new},P_{new})$\;
        }
    }
}
\Return $\emptyset$ %\mathbb{G}$
\end{algorithm}


% It takes the state space $X$, input space $U$, STL formula $\phi$, the initial state $\hat{x}_0$, the number of iterations $N$, and the user-specified stochastic robustness constraint $\kappa$\ri{Are the plant dynamics/noise diffusion matrix also inputs?}. The algorithm returns a motion plan that satisfies the constraint, if found within $N$ iterations. \qh{This part from 'It takes... ' are already written as inputs in the algorithm}

The algorithm first initializes the tree $\mathbb{G}$ with the belief of $x(0)$. Each node in this tree is a tuple $(\hat{x},P)$ of the mean and covariance of the distribution that describes the state. At every iteration, the algorithm samples a random state $\hat{x}_{rand}$ and time $t_{rand}$ and computes the nearest existing node $(\hat{x}_{near},P_{near})$. $t_{rand}$ is sampled from the time-horizon of the STL formula as defined in \cite{rosi}, and the nearest node is selected using a distance metric that accounts for both state distance $\|\hat{x}_{rand} - \hat{x}_{near}\|$ and time distance $|t_{rand} - t_{near}|$. Second, a random control input $u \in U$ and time duration $t$ is sampled and propagate the system from $(\hat{x}_{near},P_{near})$ to generate a new belief node $(\hat{x}_{new},P_{new})$. Third, the \stori Monitor of the partial belief trajectory $\ptraj = (\hat{x}_0,P_0)(\hat{x}_1,P_1)\cdots(\hat{x}_{new},P_{new})$ is computed for the formula $\phi$. If the \stori Monitor has an upper bound $\up{\Tilde{f}}(\phi,\ptraj) \leq \kappa$, $\ptraj$ has already violated the STL Specification and the new node is discarded. Otherwise, we add $(\hat{x}_{new},P_{new})$ and the edge $\big((\hat{x}_{near},P_{near}),(\hat{x}_{new},P_{new})\big)$ to $\mathbb{G}$. Finally, $\ptraj$ is a solution if the \storm $\low{f}(\phi,\ptraj) > \kappa$. This process repeats until a solution is found or for a maximum of $N$ iterations.

% We first initialize the graph with the initial state and a zero covariance matrix. At every iteration, we sample a random state $\hat{x}_{rand}$ and time $t_{rand}$ and find the nearest existing node $(\hat{x}_{near},P_{near})$. The time is sampled from the time-horizon of the STL formula \ri{how better to say this without needing definition?}, and is weighed in the distance when selecting a near node. We then sample a random control input $u \in U$ and time duration $t$ and propagate the system from $(\hat{x}_{near},P_{near})$ to generate a new belief $(\hat{x}_{new},P_{new})$. The algorithm then calculates the \stori Monitor of the partial belief trajectory $\ptraj = (\hat{x}_0,P_0)(\hat{x}_1,P_1)\cdots(\hat{x}_{new},P_{new})$ with respect to the formula $\phi$. If the \stori monitor has an upper bound $\up{\Tilde{f}}(\phi,\ptraj) < \kappa$, the partial trajectory has already violated the STL Specification and the new node is not added to the tree. Otherwise, we add the vertex $(\hat{x}_{new},P_{new})$ and the edge $[(\hat{x}_{near},P_{near}),(\hat{x}_{new},P_{new})]$ to $\mathbb{G}$. The partial trajectory is a solution if the lower bound $\low{\Tilde{f}}(\phi,\ptraj) > \kappa$. This process repeats until a solution is found or for a maximum of $N$ iterations.
% This section presents Fast Random Optimal StoRI Trees (FROST), a planning algorithm that finds motion plans for stochastic systems that satisfy a user-specified threshold on the lower bound of the StoRI of the resulting trajectory with respect to an STL formula $\phi$. \ri{I'd like to use the name GHOST if we can think of something for H (G would be 'Gaussian')}
\begin{theorem}[Probabilistic Completeness]
\label{theorem:complete}
Planner \stori-\X in Alg.~\ref{alg:StoRIX} is probabilistically complete if the underlying planner \X is probabilistically complete.
\end{theorem}
\begin{proof}[Proof]
\stori-\X mimics the behavior of planner \X, only modifying its validity check. From Theorem \ref{theorem:monitorbounds}, this modification only rejects nodes that are guaranteed to violate the STL Specification $\phi$. Therefore, if a solution exists, \stori-\X will find it with probability $1$ as $N \rightarrow \infty$. 
\end{proof}


% \ri{todo: find reach regions once at beginning of AO version}
% \begin{algorithm}[h]
% \caption{StoRI-RRT($X,U,N,\hat{x}_0,P_0,\kappa, \phi, \mathcal{R})$}
% \label{alg:RRT}
% $\mathbb{V} \gets \{(\hat{x}_0,P_0)\}$;
% $\mathbb{E} \gets \emptyset, \mathbb{G} \gets \{\mathbb{V},\mathbb{E}\}$\;
% \For{$n = 1$ to $N$}
% {
%     $t_{sample} \gets$ TimeSample($\mathbb{T}$)\;
%     $x_{sample} \gets$ ReachSample($\mathcal{R},t_{sample}$)\;
%     $x_{near} \gets$ BestNear($\mathbb{V}_{active},x_{sample},\delta v$)\;
%     $u_{sample} \gets$ SampleControl($U$)\;
%     $t_{prop} \gets$ Uniform(0,$\mathbb{T}$)\;
%     $x_{new},P_{new} \gets$ Propagate($x_{near},u_{sample},t_{prop}$)\;
%     $I \gets$ FindStoRI($x_0 \rightarrow x_{new}, \phi$)\;
%     \If{$\up{I} \geq \kappa$} {
%         $\mathbb{V} \gets \mathbb{V} \cup \{(x_{new},P_{new})\}$ \;
%         $\mathbb{E} \gets \mathbb{E} \cup \{x_{near} \rightarrow x_{new}\}$\;
%         \If{$\low{I} \geq kappa$}{
%         break\;
%         }
%     }
% }
% \Return $(\mathbb{G},n,\low{I})$\;
% \end{algorithm}



% \begin{algorithm}[h]
% \caption{FROST($X,U,\hat{x}_0,P_0,dt,N,\delta_v, \delta_s,\kappa, \phi)$}
% \label{alg:StSST}
% $i \gets 0$\;
% $\mathbb{V}_{active} \gets \{(\hat{x}_0,P_0)\}$, $\mathbb{V}_{inactive} \gets \emptyset$\;
% $\mathbb{V} \gets \mathbb{V}_{active} \cup \mathbb{V}_{inactive}$\;
% $\mathbb{E} \gets \emptyset, \mathbb{G} \gets \{\mathbb{V},\mathbb{E}\}$\;
% $s_0 \gets x_0, s_0.rep = x_0, S \gets \{s_0\}$\;
% $\mathcal{R} \gets$ FindReachRegions($\phi,\emptyset,\top,[0,0]$)\;
% \While{$N \neq 0$}
% {
%     $t_{sample} \gets$ TimeSample($\mathbb{T}$)\;
%     $s_{sample} \gets$ ReachSample($\mathcal{R},t_{sample}$)\;
%     $x_{nearest} \gets$ BestNear($\mathbb{V}_{active},s_{sample},\delta v$)\;
%     $u_{sample} \gets$ SampleControl($U$)\;
%     $x_{new} \gets$ Propagate($x_{nearest},u_{sample},dt$)\;
%     $I \gets$ FindStoRI($x_0 \rightarrow x_{new}, \phi$)\;
%     \If{$\lceil I \geq \kappa$} {
%         $s_{new} \gets$ Nearest($S,x_{new}$)\;
%         \If{$dist(x_{new},s_{new}) > \delta_s$} {
%             $S \gets S \cup \{x_{new}\}$\;
%             $s_{new} \gets x_{new}$\;
%             $s_{new}.rep \gets NULL$\;
%         }
%         $x_{peer} \gets s_{new}.rep$\;
%         \If{$x_{peer} == NULL$ or cost($x_{new}) <$ cost($x_{peer}$)} {
%             $\mathbb{V}_{active} \gets \mathbb{V}_{active} \symbol{92} \{x_{peer}\}$\;
%             $\mathbb{V}_{inactive} \gets \mathbb{V}_{inactive} \cup \{x_{peer}\}$ \;
%             $s_{new}.rep \gets x_{new}$\;
%             $\mathbb{V}_{active} \gets \mathbb{V}_{active} \cup \{x_{new}\}$ \;
%             $\mathbb{E} \gets \mathbb{E} \cup \{x_{nearest} \rightarrow x_{new}\}$\;
%             \While{IsLeaf($x_{peer}) \land x_{peer} \in \mathbb{V}_{inactive}$} {
%                 $\mathbb{E} \gets \mathbb{E} \symbol{92} \{x_{parent} \rightarrow x_{peer}\}$\;
%                 $\mathbb{V}_{inactive} \gets \mathbb{V}_{inactive} \symbol{92} \{x_{peer}\}$\; 
%                 $x_{peer} \gets x_{parent}$\;
%             }
%         }
%     }
% }
% \Return %$\mathbb{G}$\;
% \end{algorithm}

\subsection{Asymptotically Optimal StoRI-X (AO-StoRI-X)}
Since the \storm allows us to compute a quantitative value of robustness, we can also optimize for the \storm of a belief trajectory in a sampling-based motion planner. This is enabled through the AO-$\mathcal{A}$ meta-algorithm in \cite{ao-rrt}, by repeatedly calling \stori-\X with increasing $\kappa$ bounds where $\kappa$ is given as the \storm of the previous solution. 
\ri{to-do: mention how kappa is increased in AO-StoRI-X}

%%%%%%%%%%%%%%%%%
\begin{algorithm}
\caption{AO-StoRI-X($X,U,\phi,\hat{x}_0,N)$)}
\label{alg:frost}
$\kappa \gets 0$\;
\While{$N \neq 0$}{
$\btraj,n \gets $StoRI-X($X,U,\phi,\hat{x}_0,N,\kappa)$)\;
$\kappa \gets \low{f}(\phi,\btraj)$\; 
$N \gets N - n$\;
}
\Return $\btraj$ if solution found, No Solution otherwise
% \ri{do we just return the tree if we run out of time/iterations??}\qh{I think it's fine as is}
\end{algorithm}

% The algorithm is summarized in Alg.~\ref{alg:frost}.
% Here, we present Fast Robustly-Optimal StoRI Trees (FROST), a motion planner that iteratively optimizes \storm of belief trajectories. The algorithm is built upon the Asymptotically Optimal Rapidly Exploring Random Trees (AO-RRT) algorithm \cite{ao-rrt}. FROST returns the motion plan with the highest \storm for the STL formula after $N$ iterations. It repeatedly calls StoRI-X (Alg.~\ref{alg:StoRIX}) while iteratively increasing $\kappa$, optimizing the \storm of the final trajectory $\btraj$. Line $1$ of Alg.~\ref{alg:frost} initializes this robustness constraint to $0$. The algorithm first finds an initial solution using StoRI-X (line 2), with its corresponding \storm. Then, at every iteration, the algorithm sets $\kappa$ to the new found \storm of the previous solution, and finds a new solution with this new constraint.
% \begin{algorithm}
% \caption{FROST($X,U,N, M, \hat{x}_0,P_0,\phi)$)}
% \label{alg:frost}
%     $\kappa \gets 0$\;
%     % $\mathcal{R} \gets$ FindReachRegions($\phi,\emptyset,\top,[0,0]$)\;
%     $\btraj \gets $StoRI-X($X,U,M,\hat{x}_0,P_0,\kappa,\phi,\mathcal{R}$)\;
%     $\kappa \gets \low{f}(\phi,\btraj)$\;
%     \For{$N$ iterations}{
%     %\While{$N \neq 0$}{
%         $\btraj \gets $StoRI-RRT($X,U,M,\hat{x}_0,P_0,\kappa,\phi$)\;
%         $\kappa \gets \low{f}(\phi,\btraj)$\;
%         %$N \gets N - n$\;
%     }
%     \Return $\btraj$ if solution found, No Solution otherwise
% % \ri{do we just return the tree if we run out of time/iterations??}\qh{I think it's fine as is}
% \end{algorithm}
% \begin{algorithm}
% \caption{AO-StoRI-X($X,U,N,\hat{x}_0,P_0,\phi)$)}
% \label{alg:frost}
% $\kappa \gets 0$\;
% % $\mathcal{R} \gets$ FindReachRegions($\phi,\emptyset,\top,[0,0]$)\;
% $\btraj,n \gets $StoRI-X($X,U,N,\hat{x}_0,P_0,\kappa,\phi,\mathcal{R}$)\;
% $\kappa \gets \low{f}(\phi,\btraj)$\;
% $N \gets N - n$\;
% \While{$N \neq 0$}{
% $\btraj,n \gets $StoRI-RRT($X,U,N,\hat{x}_0,P_0,\kappa,\phi$)\;
% $\kappa \gets \low{f}(\phi,\btraj)$\; 
% $N \gets N - n$\;
% }
% \Return $\btraj$ if solution found, No Solution otherwise
% % \ri{do we just return the tree if we run out of time/iterations??}\qh{I think it's fine as is}
% \end{algorithm}
% \begin{proposition}[Asymptotically Optimal]
%     \label{theorem:optimal}
%     Planner AO-StoRI-X in Alg.~\ref{alg:frost} is asymptotically optimal if the underlying planner X is well-behaved. 
% \end{proposition}
% The algorithm is built upon the Asymptotically Optimal Rapidly Exploring Random Trees (AO-RRT) algorithm \cite{ao-rrt}. FROST returns the motion plan with the highest \storm for the STL formula after $N$ iterations. It repeatedly calls StoRI-X (Alg.~\ref{alg:StoRIX}) while iteratively increasing $\kappa$, optimizing the \storm of the final trajectory $\btraj$. Line $1$ of Alg.~\ref{alg:frost} initializes this robustness constraint to $0$. The algorithm first finds an initial solution using StoRI-X (line 2), with its corresponding \storm. Then, at every iteration, the algorithm sets $\kappa$ to the new found \storm of the previous solution, and finds a new solution with this new constraint.
% Therefore, we initialize $\kappa = 0.5$. \qh{this sentence still seems redundant}
%%%%%%%%%%%%%%%%%%%%%%%%% Old supplementary algos related to heuristic
% \begin{algorithm}
% \caption{FindReachRegions($\phi,\mathcal{R},reachflag,[t_1,t_2]$)}
% \label{alg:findRegions}
% \uIf{$\phi \in \{\top,\bot\}$}{
% \Return $\mathcal{R}$\;
% }
% \uElseIf{$\phi = \mu \land reachflag$}{
% \Return $\mathcal{R} \cup (\phi,[t_1,t_2])$\;
% }
% \uElseIf{$\phi = \phi_1 \land \phi_2$}{
% \uIf{IsConjunctionTree($\phi$)}{
% \uIf{$reachflag$}{
% \Return $\mathcal{R} \cup (\phi,[t_1,t_2])$\;
% }
% \uElse{
% \Return $\mathcal{R}$\;
% }
% }
% \uElse{
% FindReachRegions($\phi_1,\mathcal{R},reachflag,[t_1,t_2]$)\;
% FindReachRegions($\phi_2,\mathcal{R},reachflag,[t_1,t_2]$)\;
% }
% }
% \uElseIf{$\phi = \lnot \phi '$}{
% $reachflag = \lnot reachflag$\ri{does this make sense? flip the reach flag}\;
% FindReachRegions($\phi ',\mathcal{R},reachflag,[t_1,t_2]$)\;
% }
% \uElseIf{$\phi = \phi_1 U_{[a,b]} \phi_2$}{
% FindReachRegions($\phi_1,\mathcal{R},reachflag,[a,b]$)\;
% FindReachRegions($\phi_2,\mathcal{R},reachflag,[a,b]$)\;
% \ri{believe i need to adjust this to make sure it's correct for nested formulas as well}
% } 
% \end{algorithm}

% \begin{algorithm}
% \caption{IsConjunctionTree($\phi$)}
% \label{alg:conjTree}
% \uIf{$\phi = \phi_1 \land \phi_2$}{
% \uIf{IsConjunctionTree($\phi_1$) $\land$ IsConjunctionTree($\phi_2$)}{
% \Return $\top$\;
% }
% \uElse{
% \Return $\bot$\;
% }
% }
% \uElseIf{$\phi = \mu$}{
% \Return $\top$\;
% }
% \uElse{
% \Return $\bot$\;
% }
% \end{algorithm}

% \begin{algorithm}
% \caption{ReachSample($\mathcal{R},t$)}
% \label{alg:sample}
% \uIf{Unif$(0,1) < 0.05$ \ri{define the goal bias explicitly later}}{
% \For{$R \in \mathcal{R}$}{
% \If{$t < t_1 \lor t > t_2$}{
% $\mathcal{R} = \mathcal{R} \symbol{92} R$\;
% }
% }
% $R_{sample} =$ Unif($\mathcal{R}$)\;
% $s_{sample} = $ Unif($x \in X | x \vDash R_{sample}$)\;
% }
% \uElse{
% $s_{sample} = $ Unif($x \in X)$\;
% }
% \end{algorithm}
% \ri{try to make all functions either italicized or regular, not both}

==> sections/StoRI-Extended.tex <==
\section{Stochastic Robustness Measure}
\ri{to-do: clarify difference between stochastic trajectories and belief trajectories}
\label{sec:stori}

% \ml{DEFINED MACROs $\backslash low\{ \}$ and $\backslash up\{ \}$ for lower and upper bounds as underline and bar, respectively. USE THEM!}

\iffalse
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
     Experiment & Success Rate & average computation time (s) \\
     \hline
     Until, \stori 0.5 & 91\% & 82.98 $\pm$ 79.67 \\
     Until, \stori 0.8 & 80\% & 71.9 $\pm$ 64.45 \\
     not Until, \stori 0.5 & 89\% & 73.59 $\pm$ 76.79 \\
     not Until, \stori 0.8 & 90\% & 70.14 $\pm$ 64.49 \\
     \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
\fi

A popular method of measuring robustness of belief trajectories in motion planning is based on the notion of chance constraints \cite{blackmore2006probabilistic,luders2010chance,ho2022gaussian}. Chance constraints require that the probability of constraint violation (e.g., avoiding obstacles) not exceed some prescribed value. Motion planners typically enforce this chance constraint at each time step. 

\ri{to-do: clarify why chance constraints are not straightforward to express (timey-wimey multiple point shenanigans)} 
Such an approach is difficult to extend to STL formulas. This is primarily due to temporal operators and their time intervals. The time steps at which the chance constraints must hold are not readily apparent. Some approaches find success by generating constraints over time windows, and allocating risk of violating the constraints among time steps~\cite{C2TL,farahani2018shrinking}. However, these methods are limited to reasoning about discrete-time trajectories. This is in conflict with the fundamental idea of STL, which is expressing properties over real-valued continuous-time intervals.

Furthermore, these approaches only provide a \textit{qualitative} (boolean) judgement of a trajectory's satisfaction with respect to a chance constraint. In contrast, we seek to define a measure that provides a \textit{quantitative} judgement of a trajectory's satisfaction. This is analogous to robustness for deterministic STL that provides a quantitative measure beyond the qualitative Boolean semantics. Such a measure can then be extended to reason about partial trajectories, and hence, is advantageous for iterative methods for planning such as sampling-based tree algorithms. 

% metric:
% \begin{itemize}
%     \item QUANTITATIVE - other approaches are yes/no
%     \item "hopeful" view of partial trajectories
%     \item continuous times (small point)
% \end{itemize}

% outline:

% \begin{itemize}
%     \item difficult to extend to STL
%     \item due to temporal operators- constraint doesn't have to hold at each time step
%     \item also time windows - multiple different (equally correct) configurations to apply constraints 
%     \item methods have successfully applied chance constraints to signal temporal logic BUT (discrete time, we have no measure of the actual generated path) 
%     \item try to draw analogies to traditional STL semantics vs robustness 
%     \item opens the door for judging partial trajectories, good for iterative methods such as sampling based planners
%     \item then give intuition/etc 
%     \item then introduce StoRI
%     \item explain it, theorem, examples(?) etc
%     \item partial traces version
% \end{itemize}

% \qh{Refer to https://arxiv.org/pdf/1506.08234.pdf}
% \qh{For deterministic systems, the robustness degree is the maximum radius of the neighborhood that we can fit
% around a given signal s without changing the truth value of the formula. https://www.sciencedirect.com/science/article/pii/S0304397509004149}
% \qh{https://arxiv.org/pdf/2006.05239.pdf}

% We are interested in defining a measure that captures the essence of chance constraint. 
\ri{to-do: consider responding to: "violations sometimes means h(x(t)) < 0 but sometimes means h(x(t)) > 0}
To illustrate what such a measure might convey, consider the following example.
\begin{example}
    \label{ex:intuition}
    \emph{
    Consider the formulas $\phi_1 = \square_I \mu$ and $\phi_2 = \Diamond_I \mu$. In the case of the $\square$ operator, which states that a property must hold for all time $ t \in I$, a quantitative measure of robustness
    could be characterized by the point with the lowest probability of satisfying $\mu$ in $I$, i.e., $\min_{t\in I} P(h(\xtraj(t)) \geq 0)$, where $h$ is the linear function that $\mu$ is defined on. If the probability of violation at that point is below a certain threshold, then it is also below that threshold at every other point. Similarly, for the $\Diamond$ operator, which states that a property must hold for \textit{a} time point $ t \in I$, we could look at the point with the \textit{highest} probability of satisfying $\mu$, i.e., $\max_{t\in\langle a,b \rangle} P(h(\xtraj(t)) \geq 0)$. If the probability of violation at that point is above a certain threshold, then formula $\phi_2$ is satisfied. A quantitative measure of stochastic robustness must incorporate this conflicting treatment of temporal operators.
    }
\end{example}
This intuition guides the development of the Stochastic Robustness Interval (\stori) as defined below. 


% Consider the formula $\phi_1 = \square_{[0,10]}\lnot (\mu_1 \land \mu_2)$, which states that, for every time point between $t=0$ and $t=10$, avoid the region defined by predicates $\mu_1$ and $\mu_2$. We are interested in quantifying and constraining the point in the trajectory $\btraj$ with the highest probability of occupying the region. If this point satisfies a given constraint, then every other point also satisfies the constraint and the trajectory satisfies $\phi_1$.  

% In contrast, consider the formula $\phi_2 = \Diamond_{[0,10]} (\mu_1 \land \mu_2)$ (at any point between $t=0$ and $t=10$, reach region the region defined by predicates $\mu_1$ and $\mu_2$). We are interested in quantifying and constraining the point in the trajectory $\btraj$ with the highest probability of occupying the region. If any point satisfies a given constraint, then the trajectory is satisfies $\phi_2$. 
% For both of these formulas, we are interested in complete trajectories that are defined at all points in time in the formulas
% \ml{this sentence is unclear}
% . 

% % \qh{Don't use contractions in technical writing, see page 21 of \url{http://journals.ieeeauthorcenter.ieee.org/wp-content/uploads/sites/7/IEEE-Editorial-Style-Manual-for-Authors.pdf}}

% \ml{the following paragraph is unclear... want to say that the measure must reason over the probability bounds over linear predicates. That is because ...???}
% Furthermore, because STL is defined over predicates, we would  like to work with upper and lower bounds for the probabilities of occupying regions
% \ml{need to explain why we care about the bounds!} \ri{I feel like i do? right below this}, calculated from the probabilities of satisfying the linear predicates that define the regions. Both the upper and lower bounds are necessary; We would like to constrain the upper bound in $\phi_1$ above, but constrain the lower bound in $\phi_2$ above. This intuition guides the development of the Stochastic Robustness Interval (\stori) as defined below. 


% \ml{once active predicates is defined, then we can define the measure as follows.\\
% Given trajectory $x$, let $P(x, t, \phi)$ be the probability that point $x(t)$ on the trajectory satisfies the active predicates at time $t$. Then, the measure is defined as:
% $$f(\phi,x) = \min_{t} P(x, t, \phi)$$
% }

% \subsection{Definition}

\ri{to-do: mention remark that this is not restricted to stochastic processes, and x(t) can just be a collection of random variables}
\begin{definition}[Stochastic Robustness Interval]
    \label{def:stori}
    The Stochastic Robustness Interval (\stori) of a belief trajectory $\btraj$ over time window $[0,T]$ with respect to an STL formula $\phi$ is a functional $f(\phi, \btraj)$:
    \begin{equation*}
        f(\phi, \btraj) = [\low{f}(\phi, \btraj), \up{f}(\phi,  \btraj)]
    \end{equation*}
    such that $0 \leq \low{f}(\phi,\btraj) \leq \up{f} (\phi,\btraj) \leq 1$.  
    For a $t \in [0,T]$,
    let $\btraj^t$ be the time-shifted suffix of trajectory $\btraj$ such that %$\btraj^t(0) = \btraj(t)$ and, 
    for all $t' \in [0,T-t]$, $\btraj^t(t') = \btraj(t+t')$. 
    Then, lower bound $\low{f}(\phi,\btraj)$ and upper bound $\up{f}(\phi,\btraj)$ are recursively defined by:
    % \begin{align*}
    %     &\low{f}(\top,\btraj) &&= 1 \\
    %     &\low{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\low{f}(\lnot \phi, \btraj) &&= 1 - \up{f}(\phi,\btraj) \\
    %     &\low{f}(\phi_1 \land \phi_2, \btraj, t) &&= \max\big\{\low{f}(\phi_1,\btraj) + \low{f}(\phi_2,\btraj) -1,0\big\} \\
    %     &\low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=   
    %     \Big\{ \displaystyle \max_{t\in\langle a,b \rangle} \big\{ \max \{\low{f}(\phi_2,\btraj^t) \\
    %     & && \qquad \qquad + \min_{t'\in[0,t]}\low{f}(\phi_1,\btraj^{t'}) \} - 1,0 \big\} \Big\} 
    % \end{align*}
    % \begin{align*}
    %     &\up{f}(\top, \btraj) &&= 1 \\
    %     &\up{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\up{f}(\lnot \phi, \btraj) &&= 1 - \low{f}(\phi,\btraj) \\
    %     &\up{f}(\phi_1 \land \phi_2, \btraj, t) &&= \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\} \\
    %     &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=  \\ 
    %     \rlap{$\displaystyle \max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\} \Big\} $} \\
    % \end{align*}
    \begin{align*}
        &\low{f}(\top,\btraj) = \up{f}(\top, \btraj) = 1, \\
        &\low{f}(\mu, \btraj) = \up{f}(\mu, \btraj) = P(h(x(0)) \geq 0 ), \\
        &\low{f}(\lnot \phi, \btraj) = 1 - \up{f}(\phi,\btraj), \\
        &\up{f}(\lnot \phi, \btraj) = 1 - \low{f}(\phi,\btraj), \\
        &\low{f}(\phi_1 \land \phi_2, \btraj) = \max\big\{\low{f}(\phi_1,\btraj) + \low{f}(\phi_2,\btraj) -1,0\big\}, \\
        &\up{f}(\phi_1 \land \phi_2, \btraj) = \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\}, \\
        &\low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = \\
        & \quad \max_{t\in\langle a,b \rangle} \Big\{ \max \big\{\low{f}(\phi_2,\btraj^t) + \min_{t'\in[0,t]}\low{f}(\phi_1,\btraj^{t'}) - 1,0\big\} \Big\}, \\
        &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = \\
        & \quad \max_{t\in\langle a,b \rangle} \Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\}\Big\}.
    \end{align*}
    % \begin{align*}
    %     &\up{f}(\top, \btraj) &&= 1 \\
    %     &\up{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\up{f}(\lnot \phi, \btraj) &&= 1 - \low{f}(\phi,\btraj) \\
    %     &\up{f}(\phi_1 \land \phi_2, \btraj, t) &&= \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\} \\
    %     &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=  \\ 
    %     \rlap{$\displaystyle \max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\} \Big\} $} \\
    % \end{align*}
\end{definition}



We define the Stochastic Robustness Measure (\storm) to be the lower bound of \stori.

\begin{definition}[Stochastic Robustness Measure]
    \label{def:StochRo}
    The \emph{Stochastic Robustness Measure} (\storm) of a belief trajectory $\btraj$ with respect to STL formula $\phi$ is the lower bound of the \stori, i.e, $\low{f}(\phi, \btraj)$.
\end{definition}

The \stori is an interval that aims to quantify how robustly a belief trajectory $\btraj$ satisfies an STL formula $\phi$. The \storm of a belief trajectory is the lower bound of its \stori. 
A trajectory always satisfies a Boolean $\top$, so the \stori for $\phi = \top$ is $[1,1]$ for every trajectory. If $\phi = \mu$ is a linear predicate, both bounds of the \stori are the probability that the state at time zero $x(0)$
% \ml{this is not right... $\hat{x}(0)$ is not a random variable so the probability is either 0 or 1.}\ri{it applies to the time shifted trajectories; b(0) of the t-shifted suffix trajectory is a distribution (like think of how we check globally - shift it for every t and look at the first "0th" element)}
satisfies the linear predicate. Work \cite{blackmore2006probabilistic} \cite{pairet2021} outlines an efficient way to calculate this probability for Gaussian distributions. However, we stress that the \stori is defined for general belief distribution, and also applies to non-Gaussian beliefs. 

The \stori of the negation of a formula $\lnot \phi$ derives from the Unit Measure Axiom of Probability \cite{ProbBook}. Note that the lower bound of the \stori of $\lnot\phi$ depends on the upper bound of the \stori of $\phi$, and vice-versa. 


\begin{figure*}
\centering
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/certain.eps}
  \hfill
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/uncertain.eps}
  \hfill
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/fast_example.eps}
\caption{Sample trajectories that have a \stori of (left-to-right) $[0.72, 0.91]$, $[0.52, 0.847]$, $[0, 0]$ with respect to $\varphi_1$ in \eqref{eq:form1}}
\label{fig:examples}
\end{figure*}

The \stori for a conjunction of two formulas $\phi_1 \land \phi_2$ is inspired by the lower and upper bounds on the probability of a conjunction of two events. These are the Boole-Fr\'echet inequalities for logical conjunction \cite{frechet1935generalisation}, which make no assumptions on the independence on the events, and hence are general. Note that the measure seeks to quantify both upper and lower bounds because the upper bound is conservative when the specification seeks to enforce `avoidance' of the conjunction, but the lower bound is conservative when it seeks to enforce the `occupancy' of the conjunction. 

% The \stori for a conjunction of two formulas $\phi_1 \land \phi_2$ is inspired by the lower and upper bounds on the probability of a conjunction of two events; For any set of probabilistic events ${h_i}$, the probability of their conjunction is bounded by:
% \ri{if we keep this, should I use this general form for the equation or the simplified form for two events?}\qh{Write general form for now}
% \begin{equation}
%     \left(\sum_{i=1}^n P(h_i)\right) - n + 1 \leq P(\land_{i=1}^n h_i) \leq \min_i P(h_i)
% \end{equation}

% Because of this, the \stori of a conjunction of two predicates $f(\mu_1 \land \mu_2,\hat{\btraj})$ exactly bounds the probability that the belief at time zero satisfies both predicates $P(\hat{x}(0) \vDash \mu_1 \land \hat{x}(0) \vDash \mu_2)$. Furthermore, it provides useful quantitative information on the stochastic robustness of a trajectory when considering the conjunction of multiple formulas $f(\phi_1 \land \phi_2,\hat{\btraj})$. The \stori of a negation of a formula $\lnot \phi$ similarly derives from probability theory. 

% \ml{do we need this?  it's obvious... and also we don't have room for it}
% Logical disjunction of two formulas $\phi_1 \lor \phi_2 = \lnot (\lnot \phi_1 \land \lnot \phi_2)$. Applying the \stori to this form correctly results in the Boole-Fr\'echet inequalities for logican disjunction, i.e.,
% % \begin{equation}
% \begin{align*}
%     \low{f}(\phi_1 \lor \phi_2,\btraj) &= \max\big\{\low{f}(\phi_1,\btraj), \low{f}(\phi_2,\btraj)\}, \\
%     \up{f}(\phi_1 \lor \phi_2,\btraj) &= \min\big\{\up{f}(\phi_1,\btraj) + \up{f}(\phi_2,\btraj),1\big\}
% \end{align*}
% % \end{equation}







The \stori of $\phi_1 U_{\langle a,b \rangle} \phi_2$ is less straightforward. Intuitively, it aims to report the 
% Stochastic Robustness Measure 
\storm
at the time $t \in \langle a,b \rangle$ that best balances the point-wise probabilities that $\phi_1$ hold for all $t' \in [0,t]$ and the probability that $\phi_2$ hold at $t$. 

Note that by following Definition \ref{def:stori}, the obtained \stori for eventually and globally are: 
\begin{align}
    f(\Diamond_{\langle a,b\rangle} \phi, \btraj) &= \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\btraj^t), \; \max_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg] 
\end{align}
\begin{align}
    f(\square_{\langle a,b\rangle} \phi, \btraj) &= \bigg[\min_{t \in \langle a, b\rangle} \low{f}(\phi,\btraj^t), \; \min_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg]  
\end{align}
These intervals are fully inline with the intuition of the measure as discussed in Example~\ref{ex:intuition}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD DERIVATION (LOOKS NICE MAYBE ARXIV VERSION?
% The \stori of the temporal operator $eventually$, traditionally defined as $\Diamond_{[a,b]}\phi = \top U_{[a,b]} \phi$, is derived by considering that $f(\btraj,\top) = [1,1]$:

% \begin{align*}
%         &\low{f}(\top U_{\langle a,b \rangle} \phi, \btraj) \\ 
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \max \big\{\low{f}(\phi,\btraj^t) + \min_{t'\in[0,t]}\low{f}(\top,\btraj^{t'}) - 1,0 \big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \max \big\{\low{f}(\phi,\btraj^t) + 1 - 1,0 \big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\big\{ \low{f}(\phi,\btraj^t) \big\} \\
%         &\up{f}(\top U_{\langle a,b \rangle} \phi, \btraj)\\ 
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi,\btraj^t), \min_{t'\in[0,t]}\up{f}(\top,\btraj^{t'})\big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi,\btraj^t), 1\big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\big\{ \up{f}(\phi,\btraj^t) \big\} \\
%         &\Rightarrow f(\Diamond_{[a,b]} \phi, \btraj) = \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\btraj^t),\max_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg]  \\
% \end{align*}

% \ri{we can take out this derivation if you guys want, I feel like it's satisfying to show but we can either not show any, just show this, or I can also give quick derivations for globally and disjunction as well.}

% This agrees with the intuitively expected value presented at the beginning of this section. Similarly, the \stori of the temporal operator \textit{globally}, traditionally defined as $\square_{\langle a, b\rangle} \phi = \lnot \Diamond_{\langle a,b\rangle} \lnot \phi$, also agrees with the intuition: 

% \begin{equation*}
%     f(\square_{[a,b]} \phi, \btraj) = \bigg[\min_{t \in [a,b]} \low{f}(\phi,\btraj^t),\min_{t \in [a,b]} \up{f}(\phi,\btraj^t)\bigg]  
% \end{equation*}



% \subsection{Examples}
\begin{example}
    \label{ex:stori}
    \emph{
    % In this section, we present examples of the \stori as it relates to a couple sample trajectories. 
    Consider the environment in Fig. \ref{fig:examples} and formula
    \begin{equation}
    \label{eq:form1}
        \varphi_1 = \neg (x\geq 1 \wedge y \geq 2 \wedge x \leq 2) U_I (x \geq 3 \wedge y \geq 2),
    \end{equation}
    which specifies that the robot must avoid the obstacle until it reaches the goal at some time $t \in I$. 
    Fig. \ref{fig:examples} shows three belief trajectories, where the ellipses represent the 90\% confidence bounds of their uncertainty. 
    The first two trajectories (left and middle) have the same expectation but are subject to different amounts of process noise. 
    When evaluating against $\varphi_1$ with time interval $I = [0,6]$,
    we see both bounds of the \stori decrease
    from $[0.72, 0.91]$ for the first trajectory (left) to $[0.52, 0.85]$ for the
    the second trajectory that has more uncertainty (middle). This trajectory is less likely to clear the obstacle, and also less likely to arrive in the goal region. The third plot (right) shows the first trajectory but evaluated against $\varphi_1$ with smaller interval $I = [0, 4]$. The robot does not arrive to goal until after 5 seconds. Hence, the robot fails to satisfy the specification and its \stori is $[0, 0]$.
    }
\end{example}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

An important property of the \stori is that a trajectory which has a \storm of 1 satisfies STL formula $\phi$ with probability 1, as stated in the following theorem. 

% \subsection{Soundness} 
% The soundness of our proposed stochastic robustness interval measure is stated formally in the following theorem.

\begin{theorem}
Given belief trajectory $\btraj$ and STL formula $\phi$, if the Stochastic Robustness Measure $\low{f}(\phi,\btraj) = 1$, then every realization $\xtraj$ of $\btraj$ satisfies the specification, i.e., $\xtraj \models \phi$, except realizations on the set of measure zero.
\end{theorem}
% \qh{Prove the converse for $\up{f}(\phi,\btraj) = 0$}
\begin{proof}[Proof]
Consider any realization $\xtraj$ of $\btraj$. If $\low{f}(\phi,\btraj) = 1 \Longrightarrow (\xtraj,0) \models \phi$ and $\up{f}(\phi,\btraj) = 0 \Longrightarrow (\xtraj,0) \not\models \phi$, the \stori follows STL semantics as defined in Definition \ref{def:STLSemant}, which defines the satisfaction of a deterministic trajectory (realizations). This can be shown recursively as follows.

For boolean $\top$, the \stori of $\btraj$ trivially follows STL semantics:
\begin{align*}
    \low{f}(\top,\btraj) = 1 &\Longrightarrow (\xtraj,0) \models \top, \\
\end{align*}
For predicate $\mu$, the \stori of $\btraj$ follows STL semantics:
\begin{align*}
    \low{f}(\mu,\btraj) = 1 &\Longleftrightarrow P(h(x(0)) \geq 0 ) = 1\\
    &\Longleftrightarrow h(x(0)) \geq 0\\ %\;\forall x(0) \sim \btraj \\
    &\Longrightarrow (\xtraj,0) \models \mu,
\end{align*}
For boolean negation $\lnot \phi$, the \stori for $\btraj$ follows STL semantics:
\begin{align*}
    \low{f}(\lnot \phi,\btraj) = 1 &\Longleftrightarrow 1- \up{f}(\phi,\btraj) = 1 \\
    &\Longleftrightarrow \up{f}(\phi,\btraj) = 0 \\
    &\Longrightarrow (\xtraj,0) \not \models \phi \\
    &\Longrightarrow (\xtraj,0) \models \lnot \phi,
\end{align*}
For boolean conjunction $\phi_1 \land \phi_2$, the \stori follows STL semantics:
\begin{align*}
    \low{f}(\phi_1 \land \phi_2,\btraj) = 1 &\Longrightarrow \up{f}(\phi_1 \land \phi_2,\btraj) = 1\\
    &\Longleftrightarrow \min \big\{\low{f}(\phi_1,\btraj),\low{f}(\phi_2,\btraj)\big\} = 1\\
    &\Longleftrightarrow \low{f}(\phi_1,\btraj) = 1 \land \low{f}(\phi_2,\btraj) = 1 \\
    &\Longrightarrow (\xtraj,0) \models \phi_1 \land (\xtraj,0) \models \phi_2 \\
    &\Longrightarrow (\xtraj,0) \models (\phi_1 \land \phi_2),
\end{align*}
and finally, for temporal Until $\phi_1 U_I \phi_2$, the \stori for $\btraj$ reduces to STL semantics:
\begin{align*}
    \low{f}(\phi_1 U_I \phi_2,\btraj) = 1 &\Longrightarrow \up{f}(\phi_1 U_I \phi_2,\btraj) = 1 \\
    &\Longleftrightarrow \max_{t \in I}\Big\{\min\{\up{f}(\phi_2,\btraj^t), \\
    & \hspace{1.5cm} \min_{t' \in [0,t]}\up{f}(\phi_1,\btraj^{t'})\}\Big\} = 1 \\
    &\Longrightarrow \exists t \in I \,s.t. \min\big\{\up{f}(\phi_2,\btraj^t), \\
    & \hspace{1.5cm} \min_{t' \in [0,t]}\up{f}(\phi_1,\btraj^{t'})\big\} = 1 \\
    &\Longleftrightarrow \exists t \in I \,s.t. \Big(\up{f}(\phi_2,\btraj^t) = 1 \\
    & \hspace{1.5cm} \land \min_{t' \in [0,t]}\up{f}(\phi_1,\btraj^{t'}) = 1 \Big)\\
    &\Longrightarrow \exists t \in I \,s.t. (\xtraj,t) \models \phi_2 \\
    & \hspace{1.5cm} \land \forall t' \in [0,t]\up{f}(\phi_1,\btraj^{t'}) = 1 \\
    &\Longrightarrow \exists t \in I \,s.t. (\xtraj,t) \models \phi_2 \\
    & \hspace{1.5cm} \land \forall t' \in [0,t](\xtraj,t') \models \phi_1 \\
    &\Longrightarrow (\xtraj,0) \models (\phi_1 U_I \phi_2)
\end{align*}
Therefore, a belief trajectory $\btraj$ having a \storm of 1 with respect to STL formula $\phi$ implies that every non-zero measure realization $\xtraj$ of $\btraj$ satisfies the STL specification. 
\end{proof}



% \begin{figure}[ht]
% \centering
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/certain_example.png}
%   \caption{}
%   \label{fig:ex1} 
% \end{subfigure}
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/uncertain_example.png}
%   \caption{}
%   \label{fig:ex2}
% \end{subfigure}
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/fast_example.png}
%   \caption{}
%   \label{fig:ex3}
% \end{subfigure}
% \caption{Sample Trajectories that have a \stori of (a) [0.72,0.91], (b) [0.524,0.847], (c) [0,0] with respect to $\phi_1$}
% \end{figure}

% \begin{figure}[ht]
% \centering
%   \includegraphics[width=\linewidth]{figures/certain_example.png} 
%   \\\vspace{-5mm}
%   \includegraphics[width=\linewidth]{figures/uncertain_example.png}
%   \\\vspace{-10mm}
%   \includegraphics[width=\linewidth]{figures/fast_example.png}
%   \\\vspace{-5mm}
% \caption{Sample Trajectories that have a \stori of (top-to-bottom) [0.72,0.91], [0.524,0.847], [0,0] with respect to $\phi_1$}
% \label{fig:examples}
% \end{figure}



% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/certain_example.png}
%     \caption{Trajectory for $\phi_1$ with a \stori of [0.72,0.91]}
%     \label{fig:ex1}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/uncertain_example.png}
%     \caption{Trajectory for $\phi_1$ with a \stori of [0.52,0.85]}
%     \label{fig:ex2}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/fast_example.png}
%     \caption{Trajectory for the modified $\phi_1$ with a \stori of [0,0]}
%     \label{fig:ex3}
% \end{figure}

\subsection{\stori Monitor}

% Trajectory prefixes, though not complete, still contain behavior relevant to the satisfaction of STL formulas. Partial trajectories may reveal if a safety property has been violated or a liveliness property has been satisfied. 

\stori is defined for a given belief trajectory. It does not account for \emph{what could happen if we extend the trajectory.}
However, in some cases (such as planning), we are interested in extending trajectories to achieve a higher \storm. Hence, we need a monitor for \stori, which assumes the given trajectory is to be extended. The monitor must account for all the possible suffixes of the trajectory and how they might change the \storm. In this section, we present a monitor for the \stori with respect to a partial belief trajectory, that acts to bound the achievable \stori of any extensions of it.

\begin{definition}[StoRI Monitor]
    \label{def:Monitor}
    The Stochastic Robustness Interval (\stori) Monitor of a partial belief trajectory $\ptraj$ over time window $[0,t]$ with respect to an STL formula $\phi$ is a functional $\Tilde{f}(\phi, \ptraj)$:
    \begin{equation*}
        \Tilde{f}(\phi, \ptraj) = [\low{\Tilde{f}}(\phi, \ptraj), \up{\Tilde{f}}(\phi, \ptraj)]
    \end{equation*}
    such that $0 \leq \low{\Tilde{f}}(\phi,\ptraj) \leq \up{\Tilde{f}} (\phi,\ptraj) \leq 1$,
    where
    \begin{align*}
        &\Tilde{f}(\top,\ptraj) = f(\top,\ptraj) \\
        &\Tilde{f}(\mu,\ptraj) = f(\mu,\ptraj) \\
        &\low{\Tilde{f}}(\lnot \phi, \ptraj) = 1 - \up{\Tilde{f}}(\phi,\ptraj), \\
        &\up{\Tilde{f}}(\lnot \phi, \ptraj) = 1 - \low{\Tilde{f}}(\phi,\ptraj), \\
        &\low{\Tilde{f}}(\phi_1 \land \phi_2, \ptraj, t) = \max\big\{\low{\Tilde{f}}(\phi_1,\ptraj) + \low{\Tilde{f}}(\phi_2,\ptraj) -1,0\big\}, \\
        &\up{\Tilde{f}}(\phi_1 \land \phi_2, \ptraj, t) = \min\big\{\up{\Tilde{f}}(\phi_1,\ptraj), \up{\Tilde{f}}(\phi_2,\ptraj)\}, \\
        &\low{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) = 
        \begin{cases}
             \low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) & \text{if } t \geq a \\ 
            0 &\text{otherwise,}
        \end{cases} \\
        &\up{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) = \\ 
        &
        \begin{cases}
            \displaystyle \max \Big\{\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj), \min_{t'\in[0,b]}\up{f}(\phi_1,\ptraj^{t'})\Big\} & \text{if } t \geq 0 \\ 
            1 &\text{otherwise}
        \end{cases}
    \end{align*}
\end{definition}

The differences between the \stori and \stori Monitor arise in the temporal operators. These operators seek to bound possible future robustness, and also quantify the robustness of the behavior already seen. This is more clearly captured in the eventually and globally operators:
\begin{align}
    \Tilde{f}(\Diamond_{\langle a,b \rangle} \phi, \ptraj) &= \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\ptraj^t), \;1\bigg]  \\
    \Tilde{f}(\square_{\langle a,b \rangle } \phi, \ptraj) &= \bigg[0, \; \min_{t \in \langle a,b \rangle} \up{f}(\phi,\ptraj^t)\bigg]  
\end{align}
\ri{to-do: respond to "does [globally equation] hold for t $\leq$ b?"}
In the case of the $\square$ operator, the \stori is upper bounded by the best point in the partial trajectory, but is lower bounded by zero to account for possible future violation. In the case of the $\Diamond$ operator, the \stori is lower bounded by the best point in the partial trajectory, but is upper bounded by one to account for possible future ``perfect" satisfaction. 

The following theorem proves the correctness of \stori Monitor by showing that it always subsumes \stori.

\begin{lemma}
    \label{lemma:monitorupper}
    Let $\btraj$ be a belief trajectory over time window $[0,T]$ and $\btraj_t$ be a prefix of $\btraj$ where $t \in [0,T]$. Then, given STL formula $\phi$, the upper bound of the StoRI Monitor for $\btraj_t$ is monotonically decreasing with respect to $t$.
\end{lemma}
\begin{proof}
    The proof is provided in the Appendix. 
\end{proof}

\begin{lemma}
    \label{lemma:monitorlower}
    Let $\btraj$ be a belief trajectory over time window $[0,T]$ and $\btraj_t$ be a prefix of $\btraj$ where $t \in [0,T]$. Then, given STL formula $\phi$, the lower bound of the StoRI Monitor for $\btraj_t$ is monotonically increasing with respect to $t$.
\end{lemma}
\begin{proof}
    Without loss of generality, consider $\phi = \psi_1 U_{[a,b]} \psi_2$. From Definition \ref{def:Monitor}, the lower bound of the monitor of $\phi$ is:
    \begin{align*}
        &\low{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) = \\
        & = \low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) \\
        & = \max_{t\in\langle a,b \rangle} \Big\{ \max \big\{\low{f}(\phi_2,\ptraj^t) + \min_{t'\in[0,t]}\low{f}(\phi_1,\ptraj^{t'}) - 1,0\big\} \Big\},
    \end{align*}
    for $t \geq a$, which monotonically increases with respect to $t$. For $t \not\geq a$, the monitor takes on a value of 0. Because 0 is the lowest value the \stori Monitor can take, it will never decrease with respect to $t$. Therefore, the lower bound of the monitor monotonically increases with respect to t.
\end{proof}

\begin{lemma}
    \label{lemma:subsume}
    Let $\btraj$ be a belief trajectory over time window $[0,T]$. Then, given STL formula $\phi$, the \stori Monitor of $\btraj$ subsumes the \stori of $\btraj$.
\end{lemma}
\begin{proof}
    We show that for any belief trajectory $\btraj$, the value of the StoRI Monitor's upper bound is greater than or equal to the value of the StoRI's upper bound, i.e.,
    \begin{align*}
        &\up{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = \\
        &= \max \Big\{\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj), \min_{t'\in[0,b]}\up{f}(\phi_1,\btraj^{t'})\Big\} \\
        &\geq \up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) \hspace{1.8cm} \text{for } t \geq 0 \\
        &\text{and } \up{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = 1 \\
        &\geq \up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) \hspace{1cm} \text{for } t \not\geq 0,
    \end{align*}
    and the value of the StoRI Monitor's lower bound is less than or equal to the value of the StoRI's lower bound, i.e.,
    \begin{align*}
        &\low{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = \low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) \text{ for when } t \geq a \\
        &\low{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = 0 \leq \low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) \text{ for when } t \not\geq a
    \end{align*}
    Therefore, \stori Monitor of $\btraj$ subsumes \stori of $\btraj$.
\end{proof}

\begin{theorem}
    \label{theorem:monitorbounds}
    Let $\btraj$ be a belief trajectory over time window $[0,T]$ and $\btraj_t$ be a prefix of $\btraj$ where $t \in [0,T]$.  Then, given STL formula $\phi$, the StoRI Monitor for $\btraj_t$ subsumes the StoRI of $\btraj$ for all $t \in [0,T]$, i.e., $\forall t \in [0,T]$, $f(\phi,\btraj) \subseteq \Tilde{f}(\phi,\btraj_t)$.
\end{theorem}
\begin{proof}[Proof]
    From Lemma \ref{lemma:subsume}, when $t = T$, the \stori Monitor of $\btraj_t$ subsumes \stori of $\btraj$. From Lemmas \ref{lemma:monitorupper} and \ref{lemma:monitorlower}, for every $t < T$, the \stori Monitor of $\btraj_{t}$ subsumes the \stori Monitor of $\btraj_{T}$. Then it follows that the the \stori monitor of $\btraj_t$ subsumes the \stori of $\btraj$ for all $t \leq T$.
\end{proof}

% From definition \ref{def:Monitor}, we see that the upper bound of the \stori Monitor $\up{\Tilde{f}}(\phi,\ptraj) \geq \up{f}(\phi,\btraj)$. Similarly, the lower bound of the \stori Monitor $\low{\Tilde{f}}(\phi,\ptraj) \leq \low{f}(\phi,\btraj)$. Therefore, $f(\phi,\btraj) \subseteq \Tilde{f}(\phi,\btraj_t)$. \ri{is it that simple? feel like this isn't right}. 

\begin{example}
    \label{ex:monitor}
    \emph{
    Recall the STL formula in Example~\ref{ex:stori} and sample trajectories in Fig. \ref{fig:examples}.
    The \stori Monitor of the trajectories at different points in their evolution are shown in the plots in Fig. \ref{fig:examples}. Note that they subsume the \stori of the final trajectory and the interval gets smaller as the trajectory approaches the goal region. 
    }
\end{example}

==> sections/StoRI.tex <==
\section{Stochastic Robustness Measure}
\label{sec:stori}
\ri{to-do: clarify difference between stochastic trajectories and belief trajectories}

% \ml{DEFINED MACROs $\backslash low\{ \}$ and $\backslash up\{ \}$ for lower and upper bounds as underline and bar, respectively. USE THEM!}

\iffalse
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
     Experiment & Success Rate & average computation time (s) \\
     \hline
     Until, \stori 0.5 & 91\% & 82.98 $\pm$ 79.67 \\
     Until, \stori 0.8 & 80\% & 71.9 $\pm$ 64.45 \\
     not Until, \stori 0.5 & 89\% & 73.59 $\pm$ 76.79 \\
     not Until, \stori 0.8 & 90\% & 70.14 $\pm$ 64.49 \\
     \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
\fi

A popular method of measuring robustness of belief trajectories in motion planning is based on the notion of chance constraints \cite{blackmore2006probabilistic,luders2010chance,ho2022gaussian}. Chance constraints require that the probability of constraint violation (e.g., avoiding obstacles) not exceed some prescribed value. Motion planners typically enforce this chance constraint at each time step. 

\ri{to-do: clarify why chance constraints are not straightforward to express (timey-wimey multiple point shenanigans)} 

Such an approach is difficult to extend to STL formulas. This is primarily due to temporal operators and their time intervals. The time steps at which the chance constraints must hold are not readily apparent. Some approaches find success by generating constraints over time windows, and allocating risk of violating the constraints among time steps~\cite{C2TL,farahani2018shrinking}. However, these methods are limited to reasoning about discrete-time trajectories. This is in conflict with the fundamental idea of STL, which is expressing properties over real-valued continuous-time intervals.

Furthermore, these approaches only provide a \textit{qualitative} (boolean) judgement of a trajectory's satisfaction with respect to a chance constraint. In contrast, we seek to define a measure that provides a \textit{quantitative} judgement of a trajectory's satisfaction. This is analogous to robustness for deterministic STL that provides a quantitative measure beyond the qualitative Boolean semantics. Such a measure can then be extended to reason about partial trajectories, and hence, is advantageous for iterative methods for planning such as sampling-based tree algorithms. 

% metric:
% \begin{itemize}
%     \item QUANTITATIVE - other approaches are yes/no
%     \item "hopeful" view of partial trajectories
%     \item continuous times (small point)
% \end{itemize}

% outline:

% \begin{itemize}
%     \item difficult to extend to STL
%     \item due to temporal operators- constraint doesn't have to hold at each time step
%     \item also time windows - multiple different (equally correct) configurations to apply constraints 
%     \item methods have successfully applied chance constraints to signal temporal logic BUT (discrete time, we have no measure of the actual generated path) 
%     \item try to draw analogies to traditional STL semantics vs robustness 
%     \item opens the door for judging partial trajectories, good for iterative methods such as sampling based planners
%     \item then give intuition/etc 
%     \item then introduce StoRI
%     \item explain it, theorem, examples(?) etc
%     \item partial traces version
% \end{itemize}

% \qh{Refer to https://arxiv.org/pdf/1506.08234.pdf}
% \qh{For deterministic systems, the robustness degree is the maximum radius of the neighborhood that we can fit
% around a given signal s without changing the truth value of the formula. https://www.sciencedirect.com/science/article/pii/S0304397509004149}
% \qh{https://arxiv.org/pdf/2006.05239.pdf}

% We are interested in defining a measure that captures the essence of chance constraint. 
\ri{to-do: consider responding to: "violations sometimes means h(x(t)) < 0 but sometimes means h(x(t)) > 0}
To illustrate what such a measure might convey, consider the following example.
\begin{example}
    \label{ex:intuition}
    \emph{
    Consider the formulas $\phi_1 = \square_I \mu$ and $\phi_2 = \Diamond_I \mu$. In the case of the $\square$ operator, which states that a property must hold for all time $ t \in I$, a quantitative measure of robustness
    could be characterized by the point with the lowest probability of satisfying $\mu$ in $I$, i.e., $\min_{t\in I} P(h(\xtraj(t)) \geq 0)$, where $h$ is the linear function that $\mu$ is defined on. If the probability of violation at that point is below a certain threshold, then it is also below that threshold at every other point. Similarly, for the $\Diamond$ operator, which states that a property must hold for \textit{a} time point $ t \in I$, we could look at the point with the \textit{highest} probability of satisfying $\mu$, i.e., $\max_{t\in\langle a,b \rangle} P(h(\xtraj(t)) \geq 0)$. If the probability of violation at that point is above a certain threshold, then formula $\phi_2$ is satisfied. A quantitative measure of stochastic robustness must incorporate this conflicting treatment of temporal operators.
    }
\end{example}
This intuition guides the development of the Stochastic Robustness Interval (\stori) as defined below. 


% Consider the formula $\phi_1 = \square_{[0,10]}\lnot (\mu_1 \land \mu_2)$, which states that, for every time point between $t=0$ and $t=10$, avoid the region defined by predicates $\mu_1$ and $\mu_2$. We are interested in quantifying and constraining the point in the trajectory $\btraj$ with the highest probability of occupying the region. If this point satisfies a given constraint, then every other point also satisfies the constraint and the trajectory satisfies $\phi_1$.  

% In contrast, consider the formula $\phi_2 = \Diamond_{[0,10]} (\mu_1 \land \mu_2)$ (at any point between $t=0$ and $t=10$, reach region the region defined by predicates $\mu_1$ and $\mu_2$). We are interested in quantifying and constraining the point in the trajectory $\btraj$ with the highest probability of occupying the region. If any point satisfies a given constraint, then the trajectory is satisfies $\phi_2$. 
% For both of these formulas, we are interested in complete trajectories that are defined at all points in time in the formulas
% \ml{this sentence is unclear}
% . 

% % \qh{Don't use contractions in technical writing, see page 21 of \url{http://journals.ieeeauthorcenter.ieee.org/wp-content/uploads/sites/7/IEEE-Editorial-Style-Manual-for-Authors.pdf}}

% \ml{the following paragraph is unclear... want to say that the measure must reason over the probability bounds over linear predicates. That is because ...???}
% Furthermore, because STL is defined over predicates, we would  like to work with upper and lower bounds for the probabilities of occupying regions
% \ml{need to explain why we care about the bounds!} \ri{I feel like i do? right below this}, calculated from the probabilities of satisfying the linear predicates that define the regions. Both the upper and lower bounds are necessary; We would like to constrain the upper bound in $\phi_1$ above, but constrain the lower bound in $\phi_2$ above. This intuition guides the development of the Stochastic Robustness Interval (\stori) as defined below. 


% \ml{once active predicates is defined, then we can define the measure as follows.\\
% Given trajectory $x$, let $P(x, t, \phi)$ be the probability that point $x(t)$ on the trajectory satisfies the active predicates at time $t$. Then, the measure is defined as:
% $$f(\phi,x) = \min_{t} P(x, t, \phi)$$
% }

% \subsection{Definition}
\ri{to-do: mention remark that this is not restricted to stochastic processes, and x(t) can just be a collection of random variables}
\begin{definition}[Stochastic Robustness Interval]
    \label{def:stori}
    The Stochastic Robustness Interval (\stori) of a belief trajectory $\btraj$ over time window $[0,T]$ with respect to an STL formula $\phi$ is a functional $f(\phi, \btraj)$:
    \begin{equation*}
        f(\phi, \btraj) = [\low{f}(\phi, \btraj), \up{f}(\phi,  \btraj)]
    \end{equation*}
    such that $0 \leq \low{f}(\phi,\btraj) \leq \up{f} (\phi,\btraj) \leq 1$.  
    For a $t \in [0,T]$,
    let $\btraj^t$ be the time-shifted suffix of trajectory $\btraj$ such that %$\btraj^t(0) = \btraj(t)$ and, 
    for all $t' \in [0,T-t]$, $\btraj^t(t') = \btraj(t+t')$. 
    Then, lower bound $\low{f}(\phi,\btraj)$ and upper bound $\up{f}(\phi,\btraj)$ are recursively defined by:
    % \begin{align*}
    %     &\low{f}(\top,\btraj) &&= 1 \\
    %     &\low{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\low{f}(\lnot \phi, \btraj) &&= 1 - \up{f}(\phi,\btraj) \\
    %     &\low{f}(\phi_1 \land \phi_2, \btraj, t) &&= \max\big\{\low{f}(\phi_1,\btraj) + \low{f}(\phi_2,\btraj) -1,0\big\} \\
    %     &\low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=   
    %     \Big\{ \displaystyle \max_{t\in\langle a,b \rangle} \big\{ \max \{\low{f}(\phi_2,\btraj^t) \\
    %     & && \qquad \qquad + \min_{t'\in[0,t]}\low{f}(\phi_1,\btraj^{t'}) \} - 1,0 \big\} \Big\} 
    % \end{align*}
    % \begin{align*}
    %     &\up{f}(\top, \btraj) &&= 1 \\
    %     &\up{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\up{f}(\lnot \phi, \btraj) &&= 1 - \low{f}(\phi,\btraj) \\
    %     &\up{f}(\phi_1 \land \phi_2, \btraj, t) &&= \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\} \\
    %     &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=  \\ 
    %     \rlap{$\displaystyle \max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\} \Big\} $} \\
    % \end{align*}
    \begin{align*}
        &\low{f}(\top,\btraj) = \up{f}(\top, \btraj) = 1, \\
        &\low{f}(\mu, \btraj) = \up{f}(\mu, \btraj) = P(h(x(0)) \geq 0 ), \\
        &\low{f}(\lnot \phi, \btraj) = 1 - \up{f}(\phi,\btraj), \\
        &\up{f}(\lnot \phi, \btraj) = 1 - \low{f}(\phi,\btraj), \\
        &\low{f}(\phi_1 \land \phi_2, \btraj) = \max\big\{\low{f}(\phi_1,\btraj) + \low{f}(\phi_2,\btraj) -1,0\big\}, \\
        &\up{f}(\phi_1 \land \phi_2, \btraj) = \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\}, \\
        &\low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = \\
        & \quad \max_{t\in\langle a,b \rangle} \Big\{ \max \big\{\low{f}(\phi_2,\btraj^t) + \min_{t'\in[0,t]}\low{f}(\phi_1,\btraj^{t'}) - 1,0\big\} \Big\}, \\
        &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) = \\
        & \quad \max_{t\in\langle a,b \rangle} \Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\}\Big\}.
    \end{align*}
    % \begin{align*}
    %     &\up{f}(\top, \btraj) &&= 1 \\
    %     &\up{f}(\mu, \btraj) &&= P(\hat{x}(0) \vDash \mu) \\
    %     &\up{f}(\lnot \phi, \btraj) &&= 1 - \low{f}(\phi,\btraj) \\
    %     &\up{f}(\phi_1 \land \phi_2, \btraj, t) &&= \min\big\{\up{f}(\phi_1,\btraj), \up{f}(\phi_2,\btraj)\} \\
    %     &\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \btraj) &&=  \\ 
    %     \rlap{$\displaystyle \max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi_2,\btraj^t), \min_{t'\in[0,t]}\up{f}(\phi_1,\btraj^{t'})\big\} \Big\} $} \\
    % \end{align*}
\end{definition}



We define the Stochastic Robustness Measure (\storm) to be the lower bound of \stori.

\begin{definition}[Stochastic Robustness Measure]
    \label{def:StochRo}
    The \emph{Stochastic Robustness Measure} (\storm) of a belief trajectory $\btraj$ with respect to STL formula $\phi$ is the lower bound of the \stori, i.e, $\low{f}(\phi, \btraj)$.
\end{definition}

The \stori is an interval that aims to quantify how robustly a belief trajectory $\btraj$ satisfies an STL formula $\phi$. The \storm of a belief trajectory is the lower bound of its \stori. 
A trajectory always satisfies a Boolean $\top$, so the \stori for $\phi = \top$ is $[1,1]$ for every trajectory. If $\phi = \mu$ is a linear predicate, both bounds of the \stori are the probability that the state at time zero $x(0)$
% \ml{this is not right... $\hat{x}(0)$ is not a random variable so the probability is either 0 or 1.}\ri{it applies to the time shifted trajectories; b(0) of the t-shifted suffix trajectory is a distribution (like think of how we check globally - shift it for every t and look at the first "0th" element)}
satisfies the linear predicate. Work \cite{blackmore2006probabilistic} \cite{pairet2021} outlines an efficient way to calculate this probability for Gaussian distributions. However, we stress that the \stori is defined for general belief distribution, and also applies to non-Gaussian beliefs. 

The \stori of the negation of a formula $\lnot \phi$ derives from the Unit Measure Axiom of Probability \cite{ProbBook}. Note that the lower bound of the \stori of $\lnot\phi$ depends on the upper bound of the \stori of $\phi$, and vice-versa. 


\begin{figure*}
\centering
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/certain.eps}
  \hfill
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/uncertain.eps}
  \hfill
  \includegraphics[width=0.32\linewidth,trim={2cm 0 1.3cm 0},clip]{figures/fast_example.eps}
\caption{Sample trajectories that have a \stori of (left-to-right) $[0.72, 0.91]$, $[0.52, 0.847]$, $[0, 0]$ with respect to $\varphi_1$ in \eqref{eq:form1}}
\label{fig:examples}
\end{figure*}

The \stori for a conjunction of two formulas $\phi_1 \land \phi_2$ is inspired by the lower and upper bounds on the probability of a conjunction of two events. These are the Boole-Fr\'echet inequalities for logical conjunction \cite{frechet1935generalisation}, which make no assumptions on the independence on the events, and hence are general. Note that the measure seeks to quantify both upper and lower bounds because the upper bound is conservative when the specification seeks to enforce `avoidance' of the conjunction, but the lower bound is conservative when it seeks to enforce the `occupancy' of the conjunction. 

% The \stori for a conjunction of two formulas $\phi_1 \land \phi_2$ is inspired by the lower and upper bounds on the probability of a conjunction of two events; For any set of probabilistic events ${h_i}$, the probability of their conjunction is bounded by:
% \ri{if we keep this, should I use this general form for the equation or the simplified form for two events?}\qh{Write general form for now}
% \begin{equation}
%     \left(\sum_{i=1}^n P(h_i)\right) - n + 1 \leq P(\land_{i=1}^n h_i) \leq \min_i P(h_i)
% \end{equation}

% Because of this, the \stori of a conjunction of two predicates $f(\mu_1 \land \mu_2,\hat{\btraj})$ exactly bounds the probability that the belief at time zero satisfies both predicates $P(\hat{x}(0) \vDash \mu_1 \land \hat{x}(0) \vDash \mu_2)$. Furthermore, it provides useful quantitative information on the stochastic robustness of a trajectory when considering the conjunction of multiple formulas $f(\phi_1 \land \phi_2,\hat{\btraj})$. The \stori of a negation of a formula $\lnot \phi$ similarly derives from probability theory. 

% \ml{do we need this?  it's obvious... and also we don't have room for it}
% Logical disjunction of two formulas $\phi_1 \lor \phi_2 = \lnot (\lnot \phi_1 \land \lnot \phi_2)$. Applying the \stori to this form correctly results in the Boole-Fr\'echet inequalities for logican disjunction, i.e.,
% % \begin{equation}
% \begin{align}
%     \low{f}(\phi_1 \lor \phi_2) &= \max\big\{\low{f}(\phi_1,\btraj), \low{f}(\phi_2,\btraj)\}, \\
%     \up{f}(\phi_1 \lor \phi_2) &= \min\big\{\up{f}(\phi_1,\btraj) + \up{f}(\phi_2,\btraj),1\big\}.
% \end{align}
% % \end{equation}







The \stori of $\phi_1 U_{\langle a,b \rangle} \phi_2$ is less straightforward. Intuitively, it aims to report the 
% Stochastic Robustness Measure 
\storm
at the time $t \in \langle a,b \rangle$ that best balances the point-wise probabilities that $\phi_1$ hold for all $t' \in [0,t]$ and the probability that $\phi_2$ hold at $t$. 

Note that by following Definition \ref{def:stori}, the obtained \stori for eventually and globally are: 
\begin{align}
    f(\Diamond_{\langle a,b\rangle} \phi, \btraj) &= \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\btraj^t), \; \max_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg] 
\end{align}
\begin{align}
    f(\square_{\langle a,b\rangle} \phi, \btraj) &= \bigg[\min_{t \in \langle a, b\rangle} \low{f}(\phi,\btraj^t), \; \min_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg]  
\end{align}

These intervals are fully inline with the intuition of the measure as discussed in Example~\ref{ex:intuition}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD DERIVATION (LOOKS NICE MAYBE ARXIV VERSION?
% The \stori of the temporal operator $eventually$, traditionally defined as $\Diamond_{[a,b]}\phi = \top U_{[a,b]} \phi$, is derived by considering that $f(\btraj,\top) = [1,1]$:

% \begin{align*}
%         &\low{f}(\top U_{\langle a,b \rangle} \phi, \btraj) \\ 
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \max \big\{\low{f}(\phi,\btraj^t) + \min_{t'\in[0,t]}\low{f}(\top,\btraj^{t'}) - 1,0 \big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \max \big\{\low{f}(\phi,\btraj^t) + 1 - 1,0 \big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\big\{ \low{f}(\phi,\btraj^t) \big\} \\
%         &\up{f}(\top U_{\langle a,b \rangle} \phi, \btraj)\\ 
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi,\btraj^t), \min_{t'\in[0,t]}\up{f}(\top,\btraj^{t'})\big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\Big\{ \min \big\{\up{f}(\phi,\btraj^t), 1\big\} \Big\} \\
%         &=\max_{t\in\langle a,b \rangle}\big\{ \up{f}(\phi,\btraj^t) \big\} \\
%         &\Rightarrow f(\Diamond_{[a,b]} \phi, \btraj) = \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\btraj^t),\max_{t \in \langle a,b\rangle} \up{f}(\phi,\btraj^t)\bigg]  \\
% \end{align*}

% \ri{we can take out this derivation if you guys want, I feel like it's satisfying to show but we can either not show any, just show this, or I can also give quick derivations for globally and disjunction as well.}

% This agrees with the intuitively expected value presented at the beginning of this section. Similarly, the \stori of the temporal operator \textit{globally}, traditionally defined as $\square_{\langle a, b\rangle} \phi = \lnot \Diamond_{\langle a,b\rangle} \lnot \phi$, also agrees with the intuition: 

% \begin{equation*}
%     f(\square_{[a,b]} \phi, \btraj) = \bigg[\min_{t \in [a,b]} \low{f}(\phi,\btraj^t),\min_{t \in [a,b]} \up{f}(\phi,\btraj^t)\bigg]  
% \end{equation*}



% \subsection{Examples}
\begin{example}
    \label{ex:stori}
    \emph{
    % In this section, we present examples of the \stori as it relates to a couple sample trajectories. 
    Consider the environment in Fig. \ref{fig:examples} and formula
    \begin{equation}
    \label{eq:form1}
        \varphi_1 = \neg (x\geq 1 \wedge y \geq 2 \wedge x \leq 2) U_{[0,6]} (x \geq 3 \wedge y \geq 2),
    \end{equation}
    which specifies that the robot must avoid the obstacle until it reaches the goal at some time $t \in I$. 
    Fig. \ref{fig:examples} shows three belief trajectories, where the ellipses represent the 90\% confidence bounds of their uncertainty. 
    The first two trajectories (left and middle) have the same expectation but are subject to different amounts of process noise. 
    When evaluating against $\varphi_1$ with time interval $I = [0,6]$,
    we see both bounds of the \stori decrease
    from $[0.72, 0.91]$ for the first trajectory (left) to $[0.52, 0.85]$ for the
    the second trajectory that has more uncertainty (middle). This trajectory is less likely to clear the obstacle, and also less likely to arrive in the goal region. The third plot (right) shows the first trajectory but evaluated against $\varphi_1$ with smaller interval $I = [0, 4]$. The robot does not arrive to goal until after 5 seconds. Hence, the robot fails to satisfy the specification and its \stori is $[0, 0]$.
    }
\end{example}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

An important property of the \stori is that a trajectory which has a \storm of 1 satisfies STL formula $\phi$ with probability 1, as stated in the following theorem. 

% \subsection{Soundness} 
% The soundness of our proposed stochastic robustness interval measure is stated formally in the following theorem.

\begin{theorem}
Given belief trajectory $\btraj$ and STL formula $\phi$, if the Stochastic Robustness Measure $\low{f}(\phi,\btraj) = 1$, then every realization $\xtraj$ of $\btraj$ satisfies the specification, i.e., $\xtraj \models \phi$, except realizations on the set of measure zero.
\end{theorem}
% \qh{Prove the converse for $\up{f}(\phi,\btraj) = 0$}
\begin{proof}[Proof Sketch]
     The proof follows the recursive definition of \stori, and the fact that $\low{f}(\phi,\btraj) \leq \up{f} (\phi,\btraj)$. If $\low{f}(\mu,\btraj) = 1$, this implies that $P(h(\xtraj(0)) \geq 0) = 1$, i.e., almost every realization of the trajectory satisfies the predicate $\mu$. Since $\phi$ is recursively defined by $\top$ and $\mu$, by the recursive definition of \stori, we see that $\low{f}(\phi, \btraj) = 1$ implies that almost every realization of the trajectory satisfies $\phi$. A detailed proof is provided in the extended version of this paper \cite{Ilyes2022extended}.
\end{proof}



% \begin{figure}[ht]
% \centering
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/certain_example.png}
%   \caption{}
%   \label{fig:ex1} 
% \end{subfigure}
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/uncertain_example.png}
%   \caption{}
%   \label{fig:ex2}
% \end{subfigure}
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{figures/fast_example.png}
%   \caption{}
%   \label{fig:ex3}
% \end{subfigure}
% \caption{Sample Trajectories that have a \stori of (a) [0.72,0.91], (b) [0.524,0.847], (c) [0,0] with respect to $\phi_1$}
% \end{figure}

% \begin{figure}[ht]
% \centering
%   \includegraphics[width=\linewidth]{figures/certain_example.png} 
%   \\\vspace{-5mm}
%   \includegraphics[width=\linewidth]{figures/uncertain_example.png}
%   \\\vspace{-10mm}
%   \includegraphics[width=\linewidth]{figures/fast_example.png}
%   \\\vspace{-5mm}
% \caption{Sample Trajectories that have a \stori of (top-to-bottom) [0.72,0.91], [0.524,0.847], [0,0] with respect to $\phi_1$}
% \label{fig:examples}
% \end{figure}



% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/certain_example.png}
%     \caption{Trajectory for $\phi_1$ with a \stori of [0.72,0.91]}
%     \label{fig:ex1}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/uncertain_example.png}
%     \caption{Trajectory for $\phi_1$ with a \stori of [0.52,0.85]}
%     \label{fig:ex2}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = \linewidth]{figures/fast_example.png}
%     \caption{Trajectory for the modified $\phi_1$ with a \stori of [0,0]}
%     \label{fig:ex3}
% \end{figure}

\subsection{\stori Monitor}

% Trajectory prefixes, though not complete, still contain behavior relevant to the satisfaction of STL formulas. Partial trajectories may reveal if a safety property has been violated or a liveliness property has been satisfied. 

\stori is defined for a given belief trajectory. It does not account for \emph{what could happen if we extend the trajectory.}
However, in some cases (such as planning), we are interested in extending trajectories to achieve a higher \storm. Hence, we need a monitor for \stori, which assumes the given trajectory is to be extended. The monitor must account for all the possible suffixes of the trajectory and how they might change the \storm. In this section, we present a monitor for the \stori with respect to a partial belief trajectory, that acts to bound the achievable \stori of any extensions of it.

\begin{definition}[StoRI Monitor]
    \label{def:Monitor}
    The Stochastic Robustness Interval (\stori) Monitor of a partial belief trajectory $\ptraj$ over time window $[0,t]$ with respect to an STL formula $\phi$ is a functional $\Tilde{f}(\phi, \ptraj)$:
    \begin{equation*}
        \Tilde{f}(\phi, \ptraj) = [\low{\Tilde{f}}(\phi, \ptraj), \up{\Tilde{f}}(\phi, \ptraj)]
    \end{equation*}
    such that $0 \leq \low{\Tilde{f}}(\phi,\ptraj) \leq \up{\Tilde{f}} (\phi,\ptraj) \leq 1$,
    where
    \begin{align*}
        &\Tilde{f}(\top,\ptraj) = f(\top,\ptraj) \\
        &\Tilde{f}(\mu,\ptraj) = f(\mu,\ptraj) \\
        &\low{\Tilde{f}}(\lnot \phi, \ptraj) = 1 - \up{\Tilde{f}}(\phi,\ptraj), \\
        &\up{\Tilde{f}}(\lnot \phi, \ptraj) = 1 - \low{\Tilde{f}}(\phi,\ptraj), \\
        &\low{\Tilde{f}}(\phi_1 \land \phi_2, \ptraj, t) = \max\big\{\low{\Tilde{f}}(\phi_1,\ptraj) + \low{\Tilde{f}}(\phi_2,\ptraj) -1,0\big\}, \\
        &\up{\Tilde{f}}(\phi_1 \land \phi_2, \ptraj, t) = \min\big\{\up{\Tilde{f}}(\phi_1,\ptraj), \up{\Tilde{f}}(\phi_2,\ptraj)\}, \\
        &\low{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) = 
        \begin{cases}
             \low{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) & \text{if } t \geq a \\ 
            0 &\text{otherwise,}
        \end{cases} \\
        &\up{\Tilde{f}}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj) = \\ 
        &
        \begin{cases}
            \displaystyle \max \Big\{\up{f}(\phi_1 U_{\langle a,b \rangle} \phi_2, \ptraj), \min_{t'\in[0,b]}\up{f}(\phi_1,\ptraj^{t'})\Big\} & \text{if } t \geq 0 \\ 
            1 &\text{otherwise}
        \end{cases}
    \end{align*}
\end{definition}

The differences between the \stori and \stori Monitor arise in the temporal operators. These operators seek to bound possible future robustness, and also quantify the robustness of the behavior already seen. This is more clearly captured in the eventually and globally operators:
\begin{align}
    \Tilde{f}(\Diamond_{\langle a,b \rangle} \phi, \ptraj) &= \bigg[\max_{t \in \langle a,b \rangle} \low{f}(\phi,\ptraj^t), \;1\bigg]  \\
    \Tilde{f}(\square_{\langle a,b \rangle } \phi, \ptraj) &= \bigg[0, \; \min_{t \in \langle a,b \rangle} \up{f}(\phi,\ptraj^t)\bigg]  
\end{align}
\ri{to-do: respond to "does [globally equation] hold for t $\leq$ b?"}
In the case of the $\square$ operator, the \stori is upper bounded by the best point in the partial trajectory, but is lower bounded by zero to account for possible future violation. In the case of the $\Diamond$ operator, the \stori is lower bounded by the best point in the partial trajectory, but is upper bounded by one to account for possible future ``perfect" satisfaction. 

The following theorem proves the correctness of \stori Monitor by showing that it always subsumes \stori.

\begin{theorem}
    \label{theorem:monitorbounds}
    Let $\btraj$ be a belief trajectory over time window $[0,T]$ and $\btraj_t$ be a prefix of $\btraj$ where $t \in [0,T]$.  Then, given STL formula $\phi$, the StoRI Monitor for $\btraj_t$ subsumes the StoRI of $\btraj$ for all $t \in [0,T]$, i.e., $\forall t \in [0,T]$, $f(\phi,\btraj) \subseteq \Tilde{f}(\phi,\btraj_t)$.
\end{theorem}
\begin{proof}[Proof Sketch]
    Due to space constraints, we provide the general sketch of this proof. A detailed proof is provided in the extended version of this paper \cite{Ilyes2022extended}. Without loss of generality, consider $\phi = \psi_1 U_{[a,b]} \psi_2$. Using definitions \ref{def:Monitor} and \ref{def:stori}, the main idea of the proof comes from the fact that the upper bound is a monotonically decreasing function, and that the lower bound is a monotonically increasing function. Additionally, for a complete trajectory $\btraj$, $\up{\Tilde{f}}(\phi,\btraj) \geq \up{f}(\phi,\btraj)$ and $\low{\Tilde{f}}(\phi,\btraj) \leq \low{f}(\phi,\btraj)$.
\end{proof}

% From definition \ref{def:Monitor}, we see that the upper bound of the \stori Monitor $\up{\Tilde{f}}(\phi,\ptraj) \geq \up{f}(\phi,\btraj)$. Similarly, the lower bound of the \stori Monitor $\low{\Tilde{f}}(\phi,\ptraj) \leq \low{f}(\phi,\btraj)$. Therefore, $f(\phi,\btraj) \subseteq \Tilde{f}(\phi,\btraj_t)$. \ri{is it that simple? feel like this isn't right}. 

\begin{example}
    \label{ex:monitor}
    \emph{
    Recall the STL formula in Example~\ref{ex:stori} and sample trajectories in Fig. \ref{fig:examples}.
    The \stori Monitor of the trajectories at different points in their evolution are shown in the plots in Fig. \ref{fig:examples}. Note that they subsume the \stori of the final trajectory and the interval gets smaller as the trajectory approaches the goal region. 
    }
\end{example}

==> sections/SystemSetup.tex <==
\section{System Setup}
\label{sec:setup}

% \ml{Outline for this section:\\
% - Define the system as a linear stochastic differential equation (SDE)\\
% - Explain how to obtain point-wise state distribution as time evolves \\
% - interested in the properties of the robot with respect to a set of linear predicates\\
% - define the linear predicates\\
% - we express properties using STL\\
% - define STL syntax \\
% - given a deterministic signal, the semantics are clear (define)\\
% - when the signal is a random process, need an appropriate measure of robustness to evaluate the satisfaction \\
% - We are interested in motion planning, so the measure has to be appropriate for such algorithms \\
% - This implies we also need to define a monitor for it (CHALLENGING!)\\
% - In the next section we first propose an appropriate measure based on point-wise satisfaction, and then develop a monitor for it.  Then, we propose an algorithm that uses this measure for motion planning.  The algorithm can also optimize for the measure asymptotically.
% }



Consider a robotic system whose dynamics are described by
a linear stochastic differential equation (SDE):
% \cite{wiener} 
% \ml{clean up the description below... it should be simple... shouldn't need to define Eq (2).  
% Assume initial state is given $x(0)=x_0$.
% Then define how the mean and covariance evolve over time (see Slide 47 here: \url{https://ethz.ch/content/dam/ethz/special-interest/mavt/dynamic-systems-n-control/idsc-dam/Lectures/Stochastic-Systems/SDE.pdf}}
\begin{equation}
    \label{eq:SDE}
    dx(t) = (A x(t) + B u(t) ) dt + G dw(t),
\end{equation}
where $x \in X \subset \reals^n$ is the state, $u \in U \subset \reals^m$ is the control input,
$w(\cdot)$ is an $r$-dimensional Wiener process (Brownian motion) with diffusion matrix $Q \in \mathbb{R}^{r\times r}$ representing noise, $A \in \reals^{n\times n}$,  $B \in \reals^{n\times m}$, and $G \in \reals^{n\times r}$. 
The initial state of the robot is $x(0) = x_0$. 
The solution to the SDE in \eqref{eq:SDE} is a continuous-time Gaussian process \cite{LinSDE}, 
i.e., 
% $x(t) \sim b_t = \N(\hat{x}(t), \sigma(t))$,
$$x(t) \sim b_t = \N(\hat{x}(t) , P(t)),$$ 
where $b_t$, called the \textit{belief} of $x(t)$, is a normal distribution with mean $\hat{x}(t) \in X$ and covariance $P(t) \in \reals^{n\times n}$.  The evolution of $b_t$ is governed by:
% If the initial state is normally distributed $x_0 \sim \N(\hat{x}_0,P_0)$, then the evolution of the expectation $\hat{x}(t)$ and the covariance matrix $P(t)$ are given by:
\begin{align}
    \dot{\hat{x}}(t) &= A\hat{x}(t) + Bu(t),
    \label{eq:mean-dynamics}\\
    \dot{P}(t) &= AP(t) + P(t)A^T + GQG^T 
    \label{eq:covariance-dynamics}
\end{align}
with initial conditions $\hat{x}(0) = x_0$ and $P(0) = 0$.
Note that if, instead of a deterministic initial state, the robot has initial uncertainty described by a Gaussian distribution, the above equations still holds; Only the 
initial conditions $\hat{x}(0)$ and $P(0)$ change.

% Let $\mathbb{T} = \mathbb{R}_{\geq 0}$ be the continuous time domain. 
Let $T \in \reals_{\geq 0}$ be a time duration.
Then, given
% an initial state distribution $x_0 \sim \N(\hat{x}_0,P_0)$, and 
a controller $\mathbf{u}: [0,T] \rightarrow U$,  a \textit{belief trajectory} $\btraj$ over time window $[0,T]$ for the robotic system \eqref{eq:SDE} can be computed (predicted) using \eqref{eq:mean-dynamics} and \eqref{eq:covariance-dynamics}. 
% This trajectory is a continuous sequence of normally distributed random variables. 
An execution of this controller on the robotic system, called
a \textit{realization} or \textit{sample} of $\btraj$, is a \textit{state trajectory} $\xtraj$ over time duration $[0,T]$.

%and the expected value of this trajectory $E[\btraj] = \hat{\xtraj}$ is the \textit{mean trajectory}, and is deterministic. 
% $\btraj: \mathbb{T} \rightarrow (X,\mathbb{R}^{n\times n})$ \qh{define $\btraj$ properly}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%OLD DUSTY DESCRIPTION
% \ml{replace the following with the evolution equations for the mean and covariance of $x(t)$}
% The Wiener process has Gaussian increments such that $W({t_2}) - W({t_1}) \sim \N(0,Q\sqrt{t_2 - t_1})$
% \ri{not sure about this Q and its usage in the next couple of steps}
% % \ml{what's $Q$?}
% , where $\N(a,\Sigma)$ represents a multivariate Gaussian distribution with mean $a$ and covariance $\Sigma$. The pair $(u(\cdot),w(\cdot))$ is assumed to satisfy the Markov Property, and the stochastic process is fully observable. Such a system is captured by: 
% % \ml{shouldn't need to re-state the equation of motion. Try to come up with the expression for the covariance, given a time duration.  You may need to look at the solution of the SDE.}
% \begin{equation}
%     \label{eq:GaussEOM}
%     \dot{x}(t) = Ax(t) + Bu(t) + G\xi(t),
% \end{equation}
% where $\xi = \frac{dw}{dt}$ is Gaussian White Noise, a normally distributed vector with mean $E[\xi(t)] = 0$ and covariance $E[\xi(t)\xi^T(\tau)] = Q\cdot\delta (t-\tau)$. If the initial state $x_0 \sim \N(\hat{x}_0,P_0)$, then the mean of the state distribution evolves according to \ref{eq:GaussEOM} and the covariance evolves according to \cite{bucy2005filtering}: \ri{not sure if this is an ok citation, I don't actually have access to it}
% \begin{equation}
%     \dot{P} = AP + PA^T + GQG^T,
%     \label{eq:Pupdate}
% \end{equation}
% where $P \in \mathbb{R}^{n \times n}$
% % \ml{is this correct? Is $P$ positive definite?}
% . Let $\mathbb{T} = \mathbb{R}_{\geq 0}$ be the continuous time domain. Then, given an initial state distribution $x_0 \sim \N(\hat{x}_0,P_0)$, and a controller $\mathbf{u}: \mathbb{T} \rightarrow U$, the solution to system \ref{eq:SDE} is a \textit{belief trajectory} $\btraj: \mathbb{T} \rightarrow (X,\mathbb{R}^{n\times n})$. This trajectory is a continuous sequence of normally distributed random variables, and the expected value of this trajectory $E[\btraj] = \hat{\xtraj}$ is the \textit{mean trajectory}, and is deterministic. 

% \ml{simplify the description above... way too long and complicated...}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We are interested in properties of System  \eqref{eq:SDE} with respect to a set of \emph{linear predicates} defined in state space $X$. Let $\mathcal{H} = \{h_1,h_2,...,h_l\}$ be a given set of functions where $h_i: \mathbb{R}^n \rightarrow \mathbb{R}$ is a linear function for every $1 \leq i \leq l$. Then, the set of predicates $M = \{\mu_1,...,\mu_l\}$ is defined on $\mathcal{H}$ such that $\forall i \in \{1,...,l\}$, the Boolean values of $\mu_i:X\rightarrow \{\top,\bot\}$ is determined by the sign of function $h_i$ as:  
\begin{equation}
    \mu_i(x) = 
    \begin{cases}
        \top \text{ if } h_i(x) \geq 0 \\
        \bot \text{ if } h_i(x) < 0.
    \end{cases}
    \label{eq:preddef}
\end{equation}

To express desired properties of the robot with respect to the set of predicates $M$, we use \textit{signal temporal logic} (STL) \cite{Maler2004}. STL is a logic that allows specification of
real-time temporal properties,
% defined over real-valued continuous time, 
and is therefore well-suited for continuous-time systems such as the one in \eqref{eq:SDE}.

\begin{definition}[STL Syntax]
    \label{def:STLSyntax}
    The STL Syntax is recursively defined by:
    \begin{equation*}
        \phi := \top \mid \mu \mid \lnot \phi \mid \phi \land \phi \mid \phi \, \mathcal{U}_I \phi
    \end{equation*}
    where $\mu \in M$, and $I = \langle a,b \rangle$ is a time interval with $\langle \in \{(,[\}$, $\rangle \in \{),]\}$, $a,b \in \mathbb{R}_{\geq 0}$ and $a < b < \infty$. Notations $\top$, $\lnot$, and $\land$ are the Boolean ``true,"  ``negation,'' and ``conjunction,'' respectively, and $U$ denotes the temporal ``until'' operator. 
\end{definition}

% The boolean \textit{false} and other operators (disjunction, implication) are defined in the usual way. 
\noindent
The temporal operator \textit{eventually} ($\Diamond$) is defined as $\Diamond_{I}\phi \equiv \top \mathcal{U}_{I}\phi$ and the operator \textit{globally} is defined as $\square_{I}\phi \equiv \lnot \Diamond_{I}\lnot \phi$. 

\begin{definition}[STL Semantics]
\label{def:STLSemant}
    The semantics of STL is defined over a state trajectory realization $\xtraj$ 
    % of a belief trajectory $\btraj$ 
    at time $t$ as:
        \begin{alignat*}{2}
            (\xtraj,t) &\models \top &&\Longleftrightarrow \top \\
            (\xtraj,t) &\models \mu &&\Longleftrightarrow h(\xtraj(t)) \geq 0 \\
            (\xtraj,t) &\models \lnot \phi &&\Longleftrightarrow (\xtraj,t) \not\models \phi\\
            (\xtraj,t) &\models \phi_1 \land \phi_2 &&\Longleftrightarrow (\xtraj,t) \models \phi_1 \land (\xtraj,t) \models \phi_2\\
            (\xtraj,t) &\models \phi_1 \mathcal{U}_{\langle a,b \rangle} \phi_2 &&\Longleftrightarrow \exists t' \in \langle t+a,t+b \rangle \, s.t. \, (\xtraj,t') \models \phi_2 \\ & && \quad \ \quad \land \forall t'' \in [t,t'], \; (\xtraj,t'') \models \phi_1
        \end{alignat*}
    where $\models$ denotes satisfaction. A state trajectory $\xtraj$ satisfies an STL formula $\phi$ if $(\xtraj,0) \models \phi$. 
\end{definition}


In addition to the Boolean semantics, STL admits \textit{quantitative} semantics \cite{Lahijanian:AR-CRAS:2017}. This is traditionally defined as a robustness metric \cite{donze2010robust} based on Euclidian distance. 
This metric is well-defined for deterministic systems.
For a stochastic process such as System \eqref{eq:SDE}, however, evaluation of the satisfaction of a belief trajectory is not straightforward.  

In this work, we aim to develop an appropriate measure of robustness to evaluate the satisfaction of STL formulas by a belief trajectory. Specifically, we are interested in using this measure for robust motion planning for System \eqref{eq:SDE}. Therefore, the robustness measure must be appropriate for planning, namely sampling-based motion planning algorithms. This entails that the measure must be able to provide useful information for complete as well as partial trajectories. In the next section, we introduce such a measure. Then, we present a motion planning algorithm that asymptotically optimizes for this measure.
% we propose an appropriate measure based on a belief trajectory $\xtraj$'s point-wise satisfaction of an STL formula $\phi$, and then develop a monitor for it. Then, we propose an algorithm that uses this measure for motion planning. The algorithm asymptotically optimizes the measure of the resulting belief trajectory. 


==> sections/abstract.tex <==
\begin{abstract}
In this work, we present a novel robustness measure for continuous-time stochastic trajectories with respect to Signal Temporal Logic (STL) specifications. We show the soundness of the measure \ri{not soundness, correctness?} and develop a monitor for reasoning about partial trajectories. Using this monitor, we introduce an STL sampling-based motion planning algorithm for robots under uncertainty. Given a minimum robustness requirement, this algorithm finds satisfying motion plans; alternatively, the algorithm also optimizes for the measure.  We prove probabilistic completeness and asymptotic optimality of the motion planner, and demonstrate the effectiveness of our approach on several case studies. 
\end{abstract}
